SentenceMIM: A Latent Variable Language Model

SentenceMIM is a probabilistic auto-encoder for language data, trained with Mutual Information Machine (MIM) learning to provide a fixed length representation of variable length language observations (i.e., similar to VAE). Previous attempts to learn VAEs for language data faced challenges due to posterior collapse. MIM learning encourages high mutual information between observations and latent variables, and is robust against posterior collapse. As such, it learns informative representations whose dimension can be an order of magnitude higher than existing language VAEs. Importantly, the SentenceMIM loss has no hyper-parameters, simplifying optimization. We compare sentenceMIM with VAE, and AE on multiple datasets. SentenceMIM yields excellent reconstruction, comparable to AEs, with a rich structured latent space, comparable to VAEs. The structured latent representation is demonstrated with interpolation between sentences of different lengths. We demonstrate the versatility of sentenceMIM by utilizing a trained model for question-answering and transfer learning, without fine-tuning, outperforming VAE and AE with similar architectures.

==> 2021-04-21 - SentenceMIM/diag/model-arch-decoder.tex <==
\begin{tikzpicture}

% Define nodes


\node[latent]         (z) {$\z$};

\node[latent, right=of z]                          (xdec1) {$h^1_d$};
\node[const, above=of xdec1, yshift=-0.5cm]        (xdec1_token) {\small $\Mdec^{seq}(x^1|h^1_d)$};
\node[const, above=of xdec1, yshift=0.25cm]         (xdec1_token_) {the};
\node[latent, right=of xdec1]          (xdec2) {$h^2_d$};
\node[const, above=of xdec2, yshift=-0.5cm]        (xdec2_token) {\small $\Mdec^{seq}(x^2|h^2_d)$};
\node[const, above=of xdec2, yshift=0.25cm]        (xdec2_token_) {cat};
\node[latent, right=of xdec2]          (xdec3) {$h^3_d$};
\node[const, above=of xdec3, yshift=-0.5cm]        (xdec3_token) {\small $\Mdec^{seq}(x^3|h^3_d)$};
\node[const, above=of xdec3, yshift=0.25cm]        (xdec3_token_) {is};
\node[latent, right=of xdec3]          (xdec4) {$h^4_d$};
\node[const, above=of xdec4, yshift=-0.5cm]        (xdec4_token) {\small $\Mdec^{seq}(x^4|h^4_d)$};
\node[const, above=of xdec4, yshift=0.18cm]        (xdec4_token_) {sitting};
\node[latent, right=of xdec4]          (xdec5) {$h^5_d$};
\node[const, above=of xdec5, yshift=-0.5cm]        (xdec5_token) {\small $\Mdec^{seq}(x^5|h^5_d)$};
\node[const, above=of xdec5, yshift=0.18cm]        (xdec5_token_) {<EOT>};

\node[const, below=of xdec1, yshift=-0.5cm]        (xenc1_token) {<BOT>};
\node[const, below=of xdec2, yshift=-0.5cm]        (xenc2_token) {the};
\node[const, below=of xdec3, yshift=-0.5cm]        (xenc3_token) {cat};
\node[const, below=of xdec4, yshift=-0.5cm]        (xenc4_token) {is};
\node[const, below=of xdec5, yshift=-0.5cm]        (xenc5_token) {sitting};


% Define edges
\edge {z} {xdec1}
\edge[bend right=35] {z} {xdec2}
\edge[bend right=35] {z} {xdec3}
\edge[bend right=35] {z} {xdec4}
\edge[bend right=35] {z} {xdec5}

\draw[->, >={triangle 45}] (xdec1) -- (xdec2) node [label=above left:{GRU ~~~~}] {} ;
\draw[->, >={triangle 45}] (xdec2) -- (xdec3) node [label=above left:{GRU ~~~~}] {} ;
\draw[->, >={triangle 45}] (xdec3) -- (xdec4) node [label=above left:{GRU ~~~~}] {} ;
\draw[->, >={triangle 45}] (xdec4) -- (xdec5) node [label=above left:{GRU ~~~~}] {} ;



\edge {xdec1} {xdec1_token}
\edge {xdec2} {xdec2_token}
\edge {xdec3} {xdec3_token}
\edge {xdec4} {xdec4_token}
\edge {xdec5} {xdec5_token}

\edge {xenc1_token} {xdec1}
\edge {xenc2_token} {xdec2}
\edge {xenc3_token} {xdec3}
\edge {xenc4_token} {xdec4}
\edge {xenc5_token} {xdec5}

\end{tikzpicture}

==> 2021-04-21 - SentenceMIM/diag/model-arch-encoder.tex <==
\begin{tikzpicture}

% Define nodes

\node[latent]                          (xenc1) {$h^1_e$};
\node[const, below=of xenc1, yshift=0.5cm]        (xenc1_token) {<BOT>};
\node[latent, right=of xenc1]          (xenc2) {$h^2_e$};
\node[const, below=of xenc2, yshift=0.5cm]        (xenc2_token) {the};
\node[latent, right=of xenc2]          (xenc3) {$h^3_e$};
\node[const, below=of xenc3, yshift=0.5cm]        (xenc3_token) {cat};
\node[latent, right=of xenc3]          (xenc4) {$h^4_e$};
\node[const, below=of xenc4, yshift=0.5cm]        (xenc4_token) {is};
\node[latent, right=of xenc4]          (xenc5) {$h^5_e$};
\node[const, below=of xenc5, yshift=0.5cm]        (xenc5_token) {sitting};

\node[const, right=of xenc5]         (z) {$\Menc(\z|h^5_e)$};

% Define edges

\draw[->, >={triangle 45}] (xenc1) -- (xenc2) node [label=above left:{GRU ~~~}] {} ;
\draw[->, >={triangle 45}] (xenc2) -- (xenc3) node [label=above left:{GRU ~~~}] {} ;
\draw[->, >={triangle 45}] (xenc3) -- (xenc4) node [label=above left:{GRU ~~~}] {} ;
\draw[->, >={triangle 45}] (xenc4) -- (xenc5) node [label=above left:{GRU ~~~}] {} ;

\edge {xenc1_token} {xenc1}
\edge {xenc2_token} {xenc2}
\edge {xenc3_token} {xenc3}
\edge {xenc4_token} {xenc4}
\edge {xenc5_token} {xenc5}

\edge {xenc5} {z}

\end{tikzpicture}

==> 2021-04-21 - SentenceMIM/preamble-notations.tex <==
\newcommand{\bs}{\boldsymbol}
% comments
% \newcommand{\namedcomment}[3]{\textbf{\textcolor{#1}{#2: {#3}}}}
\newcommand{\namedcomment}[3]{}
\newcommand{\david}[1]{\namedcomment{red}{David}{#1}}
\newcommand{\micha}[1]{\namedcomment{blue}{Micha}{#1}}
\newcommand{\kevin}[1]{\namedcomment{green}{Kevin}{#1}}


% abbreviations
\newcommand{\eg}{{\em e.g.}}
\newcommand{\ie}{{\em i.e.}}
\newcommand{\vs}{{\em vs.}}
\newcommand{\etal}{{\em et al.}}
\newcommand{\cf}{{\em cf.}}


% variables
\renewcommand{\k}{{\mathrm{k}}}
\newcommand{\ki}{\k^{i}}
\newcommand{\kj}{\k^{j}}
\newcommand{\kbar}{\bar{\k}}

\renewcommand{\t}{{\bs{t}}}
\newcommand{\ti}{\t^{i}}
\newcommand{\tj}{\t^{j}}
\newcommand{\tbar}{\bar{\t}}

\newcommand{\x}{{\bs{x}}}
\renewcommand{\xi}{\x^{i}}
\newcommand{\xj}{\x^{j}}
\newcommand{\xbar}{\bar{\x}}

\newcommand{\z}{{\bs z}}

% parameters
\newcommand{\params}{{\bs \theta}}

% distributions
\newcommand{\M}{\mathcal{M}}
\newcommand{\Mmodel}{\M_{\params}}
\newcommand{\Msamp}{\M_{\mathcal{S}}}

\newcommand{\pjoint}{\mathcal{P}}
\newcommand{\pdata}{\pjoint_{\mathrm{data}}}

\newcommand{\pdec}{p}
\newcommand{\penc}{q}

\newcommand{\Mdec}{\pdec_{\params}}
\newcommand{\Menc}{\penc_{\params}}

% general
\newcommand{\TZK}{{TzK }}
\newcommand{\MIM}{{MIM }}
\newcommand{\AMIM}{{A-MIM }}
\newcommand{\VAEloss}{\mathcal{L}_\text{VAE}}
\newcommand{\VAEelbo}{\mathcal{R}_\mathrm{VAE}}
\newcommand{\MIMloss}{\mathcal{L}_\text{MIM}}
\newcommand{\AMIMloss}{\mathcal{L}_\text{A-MIM}}
\newcommand{\EAMIMloss}{\hat{\mathcal{L}}_\text{A-MIM}}
\newcommand{\EMIMloss}{\hat{\mathcal{L}}_\text{MIM}}
\newcommand{\CEloss}{\mathcal{L}_\text{CE}}
\newcommand{\AAE}{\mathcal{L}_\text{AAE}}
\newcommand{\DKL}[2]{\mathcal{D}_\text{KL}\left(#1\,\|\, #2\right)}
\newcommand{\JSD}[2]{\text{JSD}\left(#1\,\|\,#2\right)}
\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\DET}[2]{\left|\det \frac{\partial {#1}}{\partial {#2}}\right|}
\renewcommand{\H}[1]{H \left( \, #1 \, \right)}
\newcommand{\HD}[2]{H_{#1} \left( \, #2 \, \right)}
\newcommand{\CE}[2]{CE \left( \, #1 \,,\, #2 \, \right)}
\newcommand{\DETDF}[2]{ | \det \frac{\partial {#1}}{\partial {#2}} | }
\newcommand{\LDET}[2]{\log \DET{#1}{#2}}
\newcommand{\RMIM}{\mathrm{R}_{\mathrm{MIM}}}
\newcommand{\RAMIM}{\mathrm{R}_{\mathrm{MIM}}^{\penc}}
\newcommand{\RH}{\mathrm{R}_\mathrm{H}}
\newcommand{\RAH}{\mathrm{R}_\mathrm{H}^{\penc}}
\newcommand{\MELBO}{{MELBO }}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kevin's commands
\newcommand{\Pencoder}{\Menc(\z | \x)\, \Menc(\x)}
\newcommand{\Pdecoder}{\Mdec(\x | \z) \,\Mdec(\z)}
\newcommand{\Pencoderjoint}{\Menc(\x , \z)}
\newcommand{\Pdecoderjoint}{\Mdec(\x , \z)}
\newcommand{\Pmix}{\left (\Mdec(\x | \z)\, \pjoint(\z) + \Menc(\z | \x)\,
\pjoint(\x) \right )}
\newcommand{\Penc}{\Menc(\z | \x)\, \pjoint(\x)}
\newcommand{\Pdec}{\Mdec(\x | \z)\, \pjoint(\z)}
\newcommand{\Mdecjoint}{\Mdec \left(\x, \z \right)}
\newcommand{\Mencjoint}{\Menc \left(\x, \z \right)}
\newcommand{\dxz}{\mathrm{d}\x\mathrm{d}\z}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% dimensions and numbers
\newcommand{\Tdim}{T}
\newcommand{\Tdimi}{\Tdim^{i}}
\newcommand{\Zdim}{Z}
% number of knowledge domains
\newcommand{\Knum}{C}
% number of data points
\newcommand{\Dnum}{N}


==> 2021-04-21 - SentenceMIM/preamble.tex <==

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{caption}
\usepackage{subcaption}
% \usepackage{subfigure}
\usepackage{booktabs} % for professional tables

\usepackage[
        hidelinks,
        colorlinks=false,
        pdftex,
        pdfpagelabels,
        bookmarks,
        hyperindex,
        hyperfigures,
        linktoc=all,
        bookmarksnumbered=true,
        bookmarksopen=true
    ]{hyperref}
% \hypersetup{}


\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.

\usepackage[utf8]{inputenc}


\usepackage[pdftex]{graphicx}
% declare the path(s) where your graphic files are
\graphicspath{{images/}}
% and their extensions so you won't have to specify these with
% every instance of \includegraphics
\DeclareGraphicsExtensions{.pdf,.jpeg,.png}


\usepackage{algorithm}
\usepackage{algorithmic}


\usepackage{url}


% \usepackage{geometry}

% % \usepackage{color}
\usepackage[dvipsnames,table]{xcolor}

\usepackage{wrapfig}



% % correct bad hyphenation here
\hyphenation{}

\usepackage{natbib}

% diagrams
\usepackage{tikz}
\usetikzlibrary{bayesnet}

% environment to fit diagrams
\usepackage{environ}
\makeatletter
\newsavebox{\measure@tikzpicture}
\NewEnviron{scaletikzpicturetowidth}[1]{%
  \def\tikz@width{#1}%
  \def\tikzscale{1}\begin{lrbox}{\measure@tikzpicture}%
  \BODY
  \end{lrbox}%
  \pgfmathparse{#1/\wd\measure@tikzpicture}%
  \edef\tikzscale{\pgfmathresult}%
  \BODY
}
\makeatother

% support referencing external document
\usepackage{xr}

\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

% carry counters between external documents
\newcounter{docpart}
\def\savestatus{%
  \newwrite\tempfile%
  \immediate\openout\tempfile=docstatus\arabic{docpart}.dat%
  \immediate\write\tempfile{\thesection}%
  \immediate\write\tempfile{\theequation}%
  \immediate\closeout\tempfile%
}
\newcounter{olddocpart}
\def\recallstatus{%
  \setcounter{olddocpart}{\arabic{docpart}}
  \addtocounter{olddocpart}{-1}
  \newread\rtempfile%
  \openin\rtempfile=docstatus\arabic{olddocpart}.dat%
  \read\rtempfile to \tmp%
  \setcounter{section}{\tmp}
  \read\rtempfile to \tmp%
  \setcounter{equation}{\tmp}%
  \closein\rtempfile%
}

% Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage{wrapfig}
\usepackage{multirow}
\usepackage[toc,page]{appendix}

\usepackage{makecell}
\usepackage{placeins}

\usepackage{colortbl}
\definecolor{Gray}{gray}{0.9}

\usepackage{stackengine}
\usepackage{bbm}
\usepackage{arydshln}

\input{preamble-notations}



==> 2021-04-21 - SentenceMIM/sections/abstract.tex <==
\begin{abstract}
SentenceMIM is a probabilistic auto-encoder for language data, 
trained with Mutual Information Machine (MIM) learning 
to provide a fixed length representation of variable length 
language observations (\ie, similar to VAE).
Previous attempts to learn VAEs for language data faced challenges 
due to posterior collapse. MIM learning encourages high mutual 
information between observations and latent variables, 
and is robust against posterior collapse.  As such, it learns 
informative representations whose dimension can be an order of 
magnitude higher than existing language VAEs.
Importantly, the SentenceMIM loss has no hyper-parameters, simplifying optimization.
We compare sentenceMIM with VAE, and AE on multiple datasets. 
SentenceMIM yields excellent reconstruction, comparable to AEs,
with a rich structured latent space, comparable to VAEs. 
The structured latent representation is demonstrated with interpolation 
between sentences of different lengths.
We demonstrate the versatility of sentenceMIM by utilizing a trained model for
question-answering and transfer learning, without fine-tuning, outperforming 
VAE and AE with similar architectures.
\end{abstract}


==> 2021-04-21 - SentenceMIM/sections/ack.tex <==
% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.


==> 2021-04-21 - SentenceMIM/sections/conclusions.tex <==
\section{Conclusions}

This paper introduces sMIM, a new probabilistic auto-encoder for language modeling,
trained with A-MIM learning.  
% The resulting framework learns an encoder 
% that provides a continuous distribution over latent codes for a sentence,
% from which one can reconstruct, generate and interpolate sentences.
In particular, sMIM avoids posterior collapse, a challenging problem with VAEs applied to language,
which enables the use of larger latent dimensions compared to sVAE, by orders of magnitude.
% learning, sMIM learns representation with high mutual information between observations and latent codes.
While the reconstruction error is comparable to sAE, sMIM learns a latent representation with semantic structure, similar to sVAE, 
allowing for interpolation, perturbation, and sampling. In this sense, it achieves the best of both worlds: a semantically meaningful representation with high information content.
We also use the structured latent representation for a downstream question-answering task on YahooCQA with state-of-the-art results.
Importantly, the proposed framework has no hyper-parameters in the loss, greatly simplifying the optimization procedure.
In addition, sMIM benefits from a more expressive architecture, in contrast to sVAE, and demonstrates reduced susceptibility to over-fitting, compared to sAE. 
In future work, we will apply sMIM to more contemporary and powerful architectures like the Transformer.


==> 2021-04-21 - SentenceMIM/sections/experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments} \label{sec:nlp-experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Datasets} \label{sec:nlp-datasets}

\begin{table}[th]
    \centering
    \setlength{\tabcolsep}{0.2em} % for the horizontal padding
    {\small
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{l||ccccc}
 \hline
 & \multicolumn{3}{c}{Sentences} &  &  \\
 \hline
 (word level) & Train & Valid. & Test & Vocab. & \#words (avg.)  \\
 \hline \hline
PTB  & 42068 & 3370 & 3761 & 9877 & 21 $\pm$ 10 \\
Yahoo & 100K & 10K & 10K & 37165 & 76 $\pm$ 55  \\
Yelp15 & 100K & 10K & 10K & 19730 & 100 $\pm$ 51  \\
WikiText-103 & 200K & 10K & 2185 & 89247 & 115 $\pm$ 60\\
\hdashline[1pt/1pt]
Everything \textsuperscript{\textdagger} & 442067 & 33369 & 33760 & 105965 & 94 $\pm$ 60 \\
\hline
\end{tabular}
    }
    \vspace*{0.01cm}
    \caption{
    Dataset properties summary for Penn Tree Bank, %\citep{Marcus:1993:BLA:972470.972475}, 
    Yahoo Answers and Yelp15, %(cf.\ \citet{DBLP:journals/corr/YangHSB17}),
    and sampled WikiText-103. %\citep{DBLP:journals/corr/MerityXBS16}.
    Everything \textsuperscript{\textdagger} is the union of all four datasets.
    }
    \label{tab:posterior-collapse-text-datasets}
    % \vspace*{-0.3cm}
\end{table}

We show experimental results on four word level datasets
described in Table \ref{tab:posterior-collapse-text-datasets}, namely,
Penn Tree Bank \cite{Marcus:1993:BLA:972470.972475},
Yahoo Answers and Yelp15 (following \citet{DBLP:journals/corr/YangHSB17}),
and WikiText-103 \cite{DBLP:journals/corr/MerityXBS16}.
We use  the Yahoo and Yelp15 datasets of \citet{DBLP:journals/corr/YangHSB17}, 
which draw 100k samples for training, and 10k for validation and testing.
For WT103 we draw 200k samples for training, 10k for validation, and retain the original test data. 
Empty lines and headers were filtered from the WT103 data.

\subsection{Architecture and Optimization} \label{sec:nlp-architecture}

Our auto-encoder architecture (Figs.\ \ref{fig:sentence-mim-arch-decoder} and \ref{fig:sentence-mim-arch-encoder}) 
followed that proposed by \citet{DBLP:journals/corr/BowmanVVDJB15}.
As is common, we concatenated $\z$ with the input to the decoder 
(\ie, a "context", similar to \citet{he2018lagging,DBLP:journals/corr/YangHSB17,DBLP:journals/corr/BowmanVVDJB15}).
% We have found GRU to perform better than LSTM in most cases, and as such, we present GRU results here.
We use the same architecture, parameterization, and latent dimensions for both sMIM and a VAE 
variant called sVAE, for comparison. 
We also trained deterministic auto-encoders with the same architecture, called sAE,
by replacing the sampled latent code with the deterministic mean of the posterior (\ie, $\z_i = \E{\z'}{\Menc(\z'|\x_i)}$).
Effectively, the only difference between these variants is the choice of loss function. Training times for all models are similar.

For PTB we trained models with 1 layer GRU, latent space dimensions of 16D, 128D, and 512D, 
a 512D hidden state, 300D word embeddings, and 50\% embedding dropout.
We trained all models with Adam \citep{Kingma2014} with initial learning rate $lr = 10^{-3}$. 
Training took less than 30 minutes on a single TITAN Xp 12G GPU.
For Yahoo Answers, Yelp15, and WT103 we trained models with 1 layer GRU, 
latent space dimensions of 32D, 512D, 1024D, a 1024D hidden state, 512D word embeddings, 
and 50\% embedding dropout.
We trained these models with SGD \citep{pmlr-v28-sutskever13}, with initial $lr = 5.0$,
and 0.25 $L_2$ gradient clipping.
All model and optimization hyper-parameters were taken from publicly available implementation of the method proposed by \citet{DBLP:journals/corr/BowmanVVDJB15}.

In all cases we use a learning rate scheduler that scaled the learning rate by 0.25
following two/one epochs (PTB/other datasets, respectively) with no improvement in
the validation loss.
We used a mini-batch size of 20 in all cases.
Following \cite{Sutskever:2014:SSL:2969033.2969173} we feed the input in reverse 
to the encoder, such that the last hidden state in the encoder depends on the 
first word of the sentence. % in the decoder.  
% (This gave slightly better reconstruction results than with left to right order.)

We trained sVAEs with the regular ELBO, and with KL divergence annealing 
(denoted "+ kl"), where a scalar weight on the KL divergence term 
is increased from 0 to 1 over 10k mini-batches to lower the risk of posterior 
collapse
% and improve the learned models 
\citep{DBLP:journals/corr/BowmanVVDJB15}.
We use no loss manipulation heuristics in the optimization of sMIM or sAE.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{What Constitutes an Ideal Representation?} 

% % In what follows we probe the information that is conveyed by the latent code in sMIM, sVAE, and sAE. 
% Hypothetically, we argue that storing all the information content of the observations within the corresponding latent codes
% would constitute an ideal fixed-size representation, suitable to completely replace the observations for downstream tasks,  and easier to handle (\ie, being a more convenient format). 
% In addition, ideally, we would like the latent space to be 
% structured, such that semantically similar observations will have latent codes with shorter Euclidean distance. We propose that
% a compressed latent space, as measured by low information entropy, achieves such a learned representation.
% Interestingly, those ideas are also discussed in recent theory of the brain papers (\eg, \citet{Friston2010}).
% In practice, we are unlikely to capture all the information in the latent code, and in such cases a semantically structured 
% latent space will lead to semantic errors, as is shown later by perturbing the latent code.
% In what follows we explore the information content in the learned representation of the different learning frameworks,
% followed by a discussion of the structure in the learned representation.

% \david{Wrong location for this citation, but ok for now.}
% \micha{Moved to  Sec. 3.6}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Information Content in the Latent Code} \label{nlp-quantitative-results}

\begin{table}[t]
    \centering
    \scalebox{1.1}{
    \setlength{\tabcolsep}{0.2em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{l||c|c|c|c|c}
        \hline
        $\z$ dim. & Enc. Recon. $\downarrow$ & KL & Rand. Recon. & BLEU $\uparrow$ & $|\params|$ \\ \hline \hline
        % %%%%%%%%%%%%%%%%%%%%%%
        % sVAE (16) & 105.24 (0.12) & 1.6 & 109.66 (0.07) & 0.124 & 11M  \\
        % sVAE (128) & 106.72  (0.12) & 0.64 & 107.19 (0.03)  & 0.118 & 11M  \\
        % sVAE (512) & 108.52  (0.23) & 0.41  &  109.2 (0.05) & 0.116 & 12M \\
        % \hline
        % %%%%%%%%%%%%%%%%%%%%%% 
        % sAE (16) & 91.86  &  & 204.07 (0.328) & 0.348 & 11M  \\
        % sAE (128) & 67.56 &  & 199.65 (0.705)  & 0.589 & 11M  \\
        % sAE (512) & 62.08 &   & 239.28 (2.036) & 0.673 & 12M \\
        % \hline
        % %%%%%%%%%%%%%%%%%%%%%% 
        % sMIM (16) & 90.12 (0.03) &  & 362.77 (1.08)  & 0.35 & 11M \\
        % sMIM (128) & 67.35 (0.008) & & 777.48 (3.09) & 0.61 & 11M \\
        % sMIM (512) & \textbf{59.23} (0.01) & & 1139.16 (5.6) & \textbf{0.679} & 12M \\
        % \hdashline[1pt/1pt]
        % sMIM (1024) \textsuperscript{\textdagger} & \textbf{26.43} (0.0) & &  & \textbf{0.724} & 179M \\
        % %%%%%%%%%%%%%%%%%%%%%% 
        %%%%%%%%%%%%%%%%%%%%%% 
        sVAE (16) & 105.24 (0.12) & 1.6 & 105.91 (0.01) & 0.124 & 11M  \\
        sVAE (128) & 106.72  (0.12) & 0.64 & 106.89 (0.01)  & 0.118 & 11M  \\
        sVAE (512) & 108.52  (0.23) & 0.41  & 108.88  (0.01) & 0.116 & 12M \\
        \hline
        %%%%%%%%%%%%%%%%%%%%%% 
        sAE (16) & 91.86  &  & 163.9 (0.02) & 0.348 & 11M  \\
        sAE (128) & 67.56 &  & 113.61 (0.01)  & 0.589 & 11M  \\
        sAE (512) & 62.08 &   & 102.93 (0.01) & 0.673 & 12M \\
        \hline
        %%%%%%%%%%%%%%%%%%%%%% 
        sMIM (16) & 90.12 (0.03) &  & 161.037 (0.02)  & 0.35 & 11M \\
        sMIM (128) & 67.35 (0.008) & & 136.2 (0.04) & 0.61 & 11M \\
        sMIM (512) & \textbf{59.23} (0.01) & & 133.74 (0.01) & \textbf{0.679} & 12M \\
        \hdashline[1pt/1pt]
        sMIM (1024) \textsuperscript{\textdagger} & \textbf{26.43} (0.0) & &  & \textbf{0.724} & 179M \\
        %%%%%%%%%%%%%%%%%%%%%% 
        \hline
        \end{tabular}
        }
    }
      \vspace*{0.1cm}
    \caption{
    Reconstruction results for {\bf PTB} are averaged over 10 runs (stdev).
    Models\textsuperscript{\textdagger} use extra training data.
    Reconstruction with a sample $\z \sim \Menc(\z|\x)$ (Enc. Recon.) and with 
    a random sample $\z \sim \mathcal{N}(\z)$ (Rand. Recon.).
    % from a Gaussian with 0 mean and standard deviation taken from a Gaussian fitted to the latent codes (see Table\ \ref{tab:language-modelling-quantitative-entropy-fitted} in supplementary material). 
    An uninformative latent space will result in similar reconstruction values.
    see text for details.
    }
    \label{tab:language-modelling-quantitative-ptb}
    \vspace*{-0.1cm}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{1.1}{
    \setlength{\tabcolsep}{0.2em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{l||c|c|c|c|c}
        \hline
        $\z$ dim. & Enc. Recon. $\downarrow$ & KL & Rand. Recon. & BLEU $\uparrow$ & $|\params|$ \\ \hline \hline
        % %%%%%%%%%%%%%%%%%%%%%%
        % sVAE (32) + kl & 401.63 (0.01) & 31.86  & 488.24 (0.023)  & 0.274 & 40M \\
        % sVAE (512) + kl & 379.93 (0.01) & 4.19 & 395.03 (0.102) & 0.18 & 43M  \\
        % sVAE (1024) + kl & 384.85 (0.01) & 3.01  & 392.04 (0.06)  & 0.176 & 46M \\
        % \hline
        % %%%%%%%%%%%%%%%%%%%%%%
        % sAE (32) & 330.25  &  & 930.27 (1.617) & 0.388 & 40M  \\
        % sAE (512) & 228.34 &  & 1337.91 (5.435)  & 0.669 & 43M  \\
        % sAE (1024) & 222.7  &   & 1356.91 (2.872) & \textbf{0.684} & 46M \\
        % \hline
        % %%%%%%%%%%%%%%%%%%%%%% 
        % sMIM (32) & 396.34 (0.0) &  & 606.38 (1.449) & 0.309 & 40M  \\
        % sMIM (512) & 220.03 (0.0) &  & 3881.3 (11.619) & 0.673 & 43M \\
        % sMIM (1024) & \textbf{219.37} (0.0) &  & 3535.04 (7.055) & 0.676 & 46M \\
        % \hdashline[1pt/1pt]
        % sMIM (1024)\textsuperscript{\textdagger} & \textbf{199.72} (0.0) & & & \textbf{0.686} & 179M \\
        % %%%%%%%%%%%%%%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%%
        sVAE (32) + kl & 401.63 (0.01) & 31.86  & 425.92 (0.01)  & 0.274 & 40M \\
        sVAE (512) + kl & 379.93 (0.01) & 4.19 & 385.76 (0.01) & 0.18 & 43M  \\
        sVAE (1024) + kl & 384.85 (0.01) & 3.01  & 387.63 (0.01)  & 0.176 & 46M \\
        \hline
        %%%%%%%%%%%%%%%%%%%%%%
        sAE (32) & 330.25  &  & 697.316 (0.0) & 0.388 & 40M  \\
        sAE (512) & 228.34 &  & 515.75 (0.0)  & 0.669 & 43M  \\
        sAE (1024) & 222.7  &   & 503.87 (0.0) & \textbf{0.684} & 46M \\
        \hline
        %%%%%%%%%%%%%%%%%%%%%% 
        sMIM (32) & 396.34 (0.0) &  & 427.6 (0.0) & 0.309 & 40M  \\
        sMIM (512) & 220.03 (0.0) &  & 600.29 (0.0) & 0.673 & 43M \\
        sMIM (1024) & \textbf{219.37} (0.0) &  & 543.36 (0.0) & 0.676 & 46M \\
        \hdashline[1pt/1pt]
        sMIM (1024)\textsuperscript{\textdagger} & \textbf{199.72} (0.0) & & & \textbf{0.686} & 179M \\
        %%%%%%%%%%%%%%%%%%%%%%
        \hline
        \end{tabular}
        }
    }
      \vspace*{-0.1cm}
    \caption{
    Reconstruction results for {\bf Yelp15} are averaged over 10 runs.
    Models\textsuperscript{\textdagger} use extra training data
    (See Table \ref{tab:language-modelling-quantitative-yelp} for details).
    }
    \label{tab:language-modelling-quantitative-yelp}
    \vspace*{-0.1cm}
\end{table}

\begin{table}[t]
    \centering
    \scalebox{1.1}{
    \setlength{\tabcolsep}{0.2em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{l||c|c|c|c|c}
                \hline
        $\z$ dim. & Enc. Recon. $\downarrow$ & KL & Rand. Recon. & BLEU $\uparrow$ & $|\params|$ \\ \hline \hline
        % %%%%%%%%%%%%%%%%%%%%%%
        % sVAE (32) + kl & 320.06 (0.04)   & 14.33 & 365.53 (0.183)  & 0.181 & 67M  \\
        % sVAE (512) + kl & 329.2 (0.06)  & 7.09 & 350.51 (0.164)  & 0.139 & 70M  \\
        % sVAE (1024) + kl & 334.41 (0.09)  & 5.52 & 342.25 (0.073) & 0.131 & 73M \\
        % \hline
        % %%%%%%%%%%%%%%%%%%%%%%
        % sAE (32) &  293.75  &  & 643.24 (0.592) & 0.372 & 67M  \\
        % sAE (512) & 222.34 &  & 712.5 (1.369)  & 0.624 & 70M  \\
        % sAE (1024) & 326.66  &   &  443.99 (0.252) & 0.372  & 73M \\
        % \hline
        % %%%%%%%%%%%%%%%%%%%%%% 
        % sMIM (32) & 290.37 (0.01) & &  1366.19 (2.885) & 0.387 & 67M \\
        % sMIM (512) & 208.27 (0.0) & & 2703.49 (5.946) & 0.664 & 70M \\
        % sMIM (1024) & \textbf{205.81} (0.0) & & 2428.4 (9.569) & \textbf{0.669} & 73M \\
        % \hdashline[1pt/1pt]
        % sMIM (1024)\textsuperscript{\textdagger} & \textbf{178.82} (0.0) &  &  & \textbf{0.682} & 179M \\
        % %%%%%%%%%%%%%%%%%%%%%%
        %%%%%%%%%%%%%%%%%%%%%%
        sVAE (32) + kl & 320.06 (0.04)   & 14.33 & 326.21 (0.01)  & 0.181 & 67M  \\
        sVAE (512) + kl & 329.2 (0.06)  & 7.09 & 331.35 (0.01)  & 0.139 & 70M  \\
        sVAE (1024) + kl & 334.41 (0.09)  & 5.52 & 335.83 (0.01) & 0.131 & 73M \\
        \hline
        %%%%%%%%%%%%%%%%%%%%%%
        sAE (32) &  293.75  &  & 487.45 (0.0) & 0.372 & 67M  \\
        sAE (512) & 222.34 &  & 375.38 (0.0)  & 0.624 & 70M  \\
        sAE (1024) & 326.66  &   & 374.31 (0.0) & 0.372  & 73M \\
        \hline
        %%%%%%%%%%%%%%%%%%%%%% 
        sMIM (32) & 290.37 (0.01) & & 555.82 (0.0) & 0.387 & 67M \\
        sMIM (512) & 208.27 (0.0) & & 482.79 (0.01) & 0.664 & 70M \\
        sMIM (1024) & \textbf{205.81} (0.01) & & 475.16 (0.01) & \textbf{0.669} & 73M \\
        \hdashline[1pt/1pt]
        sMIM (1024)\textsuperscript{\textdagger} & \textbf{178.82} (0.0) &  &  & \textbf{0.682} & 179M \\
        %%%%%%%%%%%%%%%%%%%%%%
        \hline
        \end{tabular}
        }
    }
      \vspace*{-0.15cm}
    \caption{
    Reconstruction results for {\bf Yahoo Answers}, averaged over 10 runs.
    Models\textsuperscript{\textdagger} use extra training data
    (See Table \ref{tab:language-modelling-quantitative-yelp} for details).
    }
    \label{tab:language-modelling-quantitative-yahoo}
    \vspace*{-0.1cm}
\end{table}

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{0.2em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{l||c|c|c|c}
                \hline
        $\z$ dim. & Enc. Recon. $\downarrow$ & KL & BLEU $\uparrow$ & $|\params|$ \\ \hline \hline
        sVAE (1024) + kl & 481.66 (0.1)  & 12.65   & 0.165 & 153 M  \\
        \hline
        sMIM (1024) & 329.89 (0.02) &   & 0.571 & 153 M  \\
        \hdashline[1pt/1pt]
        sMIM (1024)\textsuperscript{\textdagger} & \textbf{313.66} (0.01) & & \textbf{0.603} & 179M \\
        \hline
        \end{tabular}
    }
     \vspace*{-0.15cm}
    \caption{
    Reconstruction results for {\bf WT103} are averaged over 10 runs.
    Models\textsuperscript{\textdagger} use extra training data.
    The superior reconstruction results of sMIM hold for longer sentences.
    }
    \label{tab:language-modelling-quantitative-wiki103}
    \vspace*{-0.1cm}
\end{table}


% We note that sentence-level text modelling entails appending an \textsc{<EOT>} token 
% to each line of text (\ie, decoder observation) during training.
% We remove the \textsc{<EOT>} token during evaluation, allowing fair PPL comparison with auto-regressive 
% models\footnote{For auto-regressive models, the standard PPL evaluation protocol treats 
% the test corpus as one long sequence. For VAEs, the standard protocol involves 
% estimation of NLL over sentences. We use this protocol for sVAE and sMIM NLL/PPL evaluation.}.

Directly estimating the mutual information (MI) between the high-dimensional categorical observations $\x$ 
and the corresponding latent codes $\z$ is computationally expensive~\citep{Hjelm2018}.
Instead, we focus here on reconstruction, which is related to MI~\citep{poole2019variational}. 
We choose the reconstruction entropy (\textit{Enc.\ Recon.}), which is the negative expected log-probability of the decoder, given a sample from the corresponding posterior.
In addition, we show the reconstruction entropy when the latent code is sampled from a Gaussian prior (\textit{Rand.\ Recon.}). 
The Gaussian has 0 mean and standard deviation fitted to the latent codes (see Table\ \ref{tab:language-modelling-quantitative-entropy-fitted} in supplementary material).
When the latent code conveys little information to the decoder, we expect Enc.\ Recon.\ and Rand.\ Recon.\ to be similar.
When the decoder utilizes highly informative latent codes, we expect Rand.\ Recon.\ to be significantly larger (\ie, worse).
% Importantly, the reconstruction entropy is bounded by perfect reconstruction of 0, 
% and so it provides us with an intuition regarding how far are we from storing all available information (\ie, unlike MI which is bounded below by having 0 information).
Finally we also show the 1-BLEU score, the fraction of words recovered in the sampled reconstruction.

Tables\ (\ref{tab:language-modelling-quantitative-ptb}-\ref{tab:language-modelling-quantitative-yahoo})
% \ref{tab:language-modelling-quantitative-wiki103} , and WT103.
show reconstruction results for PTB, Yelp15, Yahoo Answers.  
For all datasets but PTB, VAE learning with KL annealing was more effective than standard VAE learning;
due to the small size of PTB, annealing overfit.
Model sMIM (1024)\textsuperscript{\textdagger} is trained on all datasets (\ie, PTB, Yahoo Answers, Yelp15 and WT103).
The BLEU score is computed between test sentences and their reconstructed samples (higher is better), 
and $|\params|$ indicates the number of parameters in each model.

% PTB, Yelp15, and Yahoo Answers results  in 
Tables\ (\ref{tab:language-modelling-quantitative-ptb}-\ref{tab:language-modelling-quantitative-yahoo}) 
show that sMIM outperforms sVAE in reconstruction and BLEU score, and is comparable to sAE.
In addition, the reconstruction of sMIM and sAE improves with more latent dimensions, showing that more information is captured by the latent codes, 
whereas sVAE shows the opposite trend due to posterior collapse (\ie, encoder and random reconstructions are similar).
Notice that sAE is more susceptible to over-fitting, as is evident in Table\ \ref{tab:language-modelling-quantitative-yahoo}.
WT103 results in Table\ \ref{tab:language-modelling-quantitative-wiki103} show that the superior reconstruction of sMIM also holds with longer sentences.

In summary, sMIM shows improved performance with more expressive architecture (higher latent dimension here), 
similar to sAE, while sVAE deteriorates due to posterior collapse.
This suggests that sMIM could benefit from more powerful architectures like Transformers~\citep{Vaswani2017}, without the need for posterior collapse-mitigating heuristics.
% This suggests that using SOTA architectures, like Transformers, could benefit sMIM, 
% importantly without the need for optimization heuristics which are required to mitigate posterior collapse
% in sVAE.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Posterior Collapse in VAE} \label{sec:nlp-posterior-collapse-ptb}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.5\columnwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{images/ptb-dist/log_p_x_given_z.pdf}
        \caption{$\log \Mdec(\x_i|\z_j)$ histograms.}     
        \label{fig:nlp-dist-ptb-log_p_x_given_z}
    \end{subfigure}%
    % \vspace*{0.21cm}
    \begin{subfigure}[t]{0.5\columnwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{images/ptb-dist/log_q_z_given_x.pdf}
        \caption{$\log \Menc(\z_i|\x_j)$ histograms.}     
        \label{fig:nlp-dist-ptb-log_q_z_given_x}
    \end{subfigure}
     \vspace*{-0.25cm}
    \caption{
    Histograms of log probabilities of test data for sMIM  and 
    sVAE trained on \textbf{PTB}: Overlap between  curves indicates
    potential for poor reconstruction of input sentences.
    (a) Histograms of $\log \Mdec(\x_i|\z_j)$ for $\z_j \sim \Menc(\z|\x_j)$ when $i=j$ 
    (same input), and when $i\neq j$ (when $\x_i$ is evaluated with the 
    decoder distribution from a latent code associated with a different input sentence).
    (b) Histograms of $\log \Menc(\z_i |\x_j)$ for  $\z_i\sim\Menc(\z |\x_i)$, 
    when conditioned on the same input $i = j$, or a different input $i\neq j$.
    \label{fig:nlp-dist-ptb}
    }
    \vspace*{-0.5cm}
\end{figure}

The performance gap between sMIM and sVAE  with identical architectures is due in part to posterior collapse in VAEs 
(\ie, optimization is likely to have a role too), 
where the encoder has high posterior variance over latent codes, and hence low mutual information
(cf.\ \citep{Zhao_Song_Ermon_2018,DBLP:journals/corr/abs-1711-00464}); it coincides with the KL divergence term in the 
usual ELBO approaching zero in some or all dimensions. 
In such cases, different sentences are mapped to similar regions of the latent space (see Fig.\ \ref{fig:nlp-dist-ptb}, bottom).

% A code $\z_i \sim \Menc(\z|\x_i)$ may have high probability density under the posterior
% given a different observation, \ie, $\Menc(\z|\x_j)$ where $i\neq j$.
% In such cases, one might expect that observations sampled from $\Mdec(\x|\z_i)$,
% might have high probability under the decoder for a
% different observation, \ie, $\Mdec(\x|\z_j)$, where 
% $i\neq j$.
In contrast, given the high mutual information and reconstruction quality of sMIM, 
we only expect high decoding probability of a sentence when a latent code is sampled from
the corresponding posterior.
% we only expect high encoder and decoder densities when $i = j$.
In other words, for sMIM, the posterior variances for different input sequences
are relatively small compared
to the distance between the posterior means (Fig.\ \ref{fig:nlp-dist-ptb}, top),
allowing for accurate reconstruction.

% The histograms in Fig.\ \ref{fig:nlp-dist-ptb} illustrate this using the best 
% sMIM and sVAE models trained on PTB.
% Histograms are labeled $[i \neq i]$ and $[i=j]$ for the two cases described above.
% They show that samples generated by sMIM given one input sentence are extremely 
% unlikely to be generated from sMIM given a different sentence. 
% This is not the case for sVAE, where the histograms overlap.
% In other words, sMIM effectively maps sentences to non-overlapping regions of 
% the latent space, allowing good reconstruction. By comparison, with sVAE 
% sentences are mapped to overlapping regions of the latent space, which hinders 
% accurate reconstruction.

The issue of posterior collapse becomes harder to mitigate as the dimension of the latent space increases, because the decoder becomes more expressive.
As a consequence, language VAEs are typically limited to 32 dimensions or fewer (\eg, \citet{he2018lagging}), with only a few exceptions, such as \citet{Guu2017GeneratingSB} which opted for 128 dimensions in a very particular problem settings.  
% \citep{bosc-vincent-2020-sequence}. 
On the other hand, sMIM can easily scale up the latent dimension without issue.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Structure in the Latent Space} \label{sec:nlp-mim-vs-ae}

\begin{figure}[t]
    \vspace*{0.1cm}
    \centering
        \includegraphics[width=1.0\columnwidth]{images/latent-structure.pdf}
        \vspace*{-0.8cm}
    \caption{
    \textbf{Top:} level-sets of a 2D data distribution (\ie, GMM with 2 modes).
    Red/green dots are samples.
    \textbf{Bottom:} the corresponding variance of the posterior, per sample, 
    for MIM and VAE, and the corresponding mapping for AE. 
    A semantically structured latent space will map latent samples from the same mode closer. A collapsed posterior (\ie, VAE), might mix nearby modes, 
    whereas MIM will have smaller posterior variance due to higher MI.
    A high entropy in the AE latent space might lead to non-semantic structure, where a perturbed red latent code might be reconstructed to the green mode, in contrast to MIM.
    \label{fig:latent-structure}
    }
\end{figure}


\begin{table}[t]
    % \vspace*{-0.2cm}
    \centering
    \scalebox{1.05}{
    \setlength{\tabcolsep}{0.2em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{l||r|r|r|r}
        % & \multicolumn{4}{c}{NN empirical entropy} \\
        % \hline
        Dataset ($\z$ dim.) & \multicolumn{1}{c|}{sMIM} & \multicolumn{1}{c|}{$\mathcal{N}$} & \multicolumn{1}{c|}{sVAE} & \multicolumn{1}{c}{sAE}   \\ \hline \hline
        PTB (16D) & 11.54 [ 0.67 ]  & 22.7 & 23.04  [ 1.02 ]  & 35.95  [ 1.18 ]  \\
                %   & [ 17.22 / 0.5 ] &  &  [ 22.51 / 0.97 ] &  [ 30.49 / 2.64 ]  \\
        % \hline
        PTB (128D) &  53.73 [ 0.55 ]  & 181.62 & 225.41 [ 1.24 ]  & 259.34 [ 1.26  ]  \\
                %   &  [ 97.39 / 0.26 ] &  & [ 181.29 / 0.99 ] & [ 206.22 / 1.46 ] \\
        % \hline
        \hline
        Yelp15 (32D) & 32.22 [ 0.85 ]  & 45.4 & 50.01 [ 1.08 ]  & 73.03 [ 1.23 ]   \\
                    %  & [ 38.06 / 0.63 ] &  &  [46.31 / 1.05] & [ 59.16 / 0.99 ]  \\
        % \hline
        Yelp15 (512D) &  186.18 [ 0.56 ] & 726.49 & 994.3 [ 1.37 ] & 917.0 [ 1.3 ] \\
                    %   &  [ 333.45 / 0.21 ] &  & [ 726.15 / 0.99 ] & [ 705.14 / 0.91 ] \\
        % \hline
        \hline
        Yahoo (32D) & 23.61 [ 0.73 ] & 45.4 & 44.45 [ 1.03 ] & 76.21 [ 1.26 ]   \\
                    % &  [ 32.13 / 0.43 ] &  & [43.3 / 0.87 ] & [ 60.45 / 2.56 ]  \\
        % \hline
        Yahoo (512D) &  155.47 [ 0.48 ] & 726.49 & 991.85 [ 1.37 ] & 1003.26 [ 1.35 ] \\
                    %  &  [ 326.17 / 0.2 ] &  &  [ 724.75 / 0.99 ] & [ 744.24 / 1.07 ] \\
        \end{tabular}
        }
    }
    \vspace*{-0.1cm}
    \caption{
    Empirical entropy of the latent codes, estimated with a NN entropy estimator.
    % for sMIM, sVAE, and sAE (estimated with a NN entropy estimator).% \citet{PhysRevE.69.066138}).
    For comparison, column $\mathcal{N}$ shows the entropy of a standard Normal in $\mathbb{R}^{d}$ of corresponding latent dimension.
    In brackets is the ratio of the NN entropy to the entropy of an isotropic Gaussian fit to the latent codes.
    Ratios below 1 indicate that the latent codes are more clustered than a Gaussian, suggesting the low entropy for sMIM is not a simple consequence of down-scaling the latent codes.
    % In brackets is the entropy of a isotropic Gaussian fitted to the latent codes, and the corresponding average standard deviation [ entropy / stdev ].
    % Our goal here is to rule out simple down-scaling as the cause for the low entropy in sMIM.
    % A fitted Gaussian entropy larger than the NN entropy means that the lower NN entropy is clustered and not merely scaled, as is evident by the corresponding standard deviation.
    }
    \label{tab:language-modelling-quantitative-entropy}
    \vspace*{-0.3cm}
\end{table}

% \begin{table}[t]
%     \centering
%     \setlength{\tabcolsep}{0.2em} % for the horizontal padding
%     \scriptsize
%     \renewcommand{\arraystretch}{1.2}% for the vertical padding
%         \begin{tabular}{l||ccc|ccc}
%                 \hline
%         Data & sMIM (S) & sMIM (M) & sMIM (L)& sAE (S) & sAE (M) & sAE (L) \\ \hline \hline
%         PTB & 0.35  & 0.61 & \textbf{0.679} & 0.348  & 0.589 & 0.637  \\
%         Yelp15 & 0.309  & 0.673 & 0.676 & 0.402  & 0.682 & \textbf{0.697} \\
%         Yahoo & 0.387  & 0.664 & \textbf{0.669} & 0.395  & 0.647 & 0.394 \\
%                 \hline
%         \end{tabular}
%     \vspace*{-0.1cm}
%     \caption{
%     BLEU results for reconstruction of sMIM and AE. sMIM
%     demonstrates empirical robustness to over-fitting, when compared to sAE.
%     (S,M,L) latent dimensions corresponds to (16D, 128D, 512D) in PTB and (32D, 512D, 1024D) in Yelp15 and Yahoo Answers.
%     }
%     \label{tab:language-modelling-quantitative-bleu}
%     \vspace*{-0.1cm}
% \end{table}


Here, we explore the structure in the learned representation.
Table\ \ref{tab:language-modelling-quantitative-entropy} shows the empirical entropy, estimated using NN entropy estimator \citet{PhysRevE.69.066138}, of the latent codes for 
sMIM, sVAE, and sAE. Notice how the representation learned by sMIM has a significantly lower entropy.
We note that sVAE is regularized to match a Gaussian, which is known to introduce smoother structure into the learned representation (see discussion by \citet{bosc-vincent-2020-sequence}).
% , at the expense of susceptibility for posterior collapse.

With sMIM, we propose the use of information entropy minimization as an alternative regularization, 
which introduces meaningful structure without suffering from posterior collapse (see schematic plot in Fig.\ \ref{fig:latent-structure}).
Interestingly, neuroscientists have proposed that entropy minimization is an organizing principle in neural representations and information processing in the brain. 
Entropy minimization is viewed as allowing the agent to learn better to predict likely events \citep{Friston2010, Barlow1972}, 
compression/redundancy elimination \citep{Barlow1961},
and in terms of efficiency in energy consumption \citep{10.3389/fncom.2019.00086}.

By scaling the latent codes to reduce the variance of the aggregate posterior one can trivially reduce entropy with no benefit in terms of latent structure.
To test whether this might be the case, we also fit an isotropic Gaussian to the latent codes
(see Table\ \ref{tab:language-modelling-quantitative-entropy-fitted} in supplementary materials), 
and show the ratio between the NN entropy and the fitted entropy in brackets.
A ratio smaller than 1 suggests that the empirical entropy is more clustered than a Gaussian.
Table\ \ref{tab:language-modelling-quantitative-entropy} clearly shows that the lower empirical 
entropy cannot be explained by the scaling alone.
We attribute the gap between the fitted and empirical entropies to clustering in the latent space,  
which MIM learning empirically demonstrates \citep{2019arXiv191003175L}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reconstruction, Interpolation, and Perturbation} \label{sec:nlp-recon}

% \begin{table}[ht]
%     \centering
%     \setlength{\tabcolsep}{0.5em} % for the horizontal padding
%     {\scriptsize
%     \renewcommand{\arraystretch}{1.2}% for the vertical padding
%         \begin{tabular}{p{8cm}}
%         \textbf{5 stars $\rightarrow$ 1 stars} \\ \hline \hline
%         \rowcolor{Gray}
% \textsc{<BOT>} awesome food , just awesome ! top notch beer selection . great staff . beer garden is great setting . \\

% \hline

% \textbullet ~ awesome food , just top notch ! great beer selection . staff has great craft beer . top notch is that . \textsc{<EOT>} \\

% \textbullet ~ awesome food , just so-so ! great beer selection . staff is top notch . great beer selection . \textsc{<EOT>} \\


% \textbullet ~ awesome food ! beer selection is just ok , not great . staff on top notch hand sanitizer . \textsc{<EOT>} \\


% \textbullet ~ cleanliness is awesome ! not only on their game , food . server was polite his hand sanitizer outside . \textsc{<EOT>} \\

% \textbullet ~ cleanliness is not on their patio . server was inattentive , kept running outside his hand sanitizer  \textsc{<EOT>} \\

% \textbullet ~ cleanliness is not on their patio . server was outside , kept running his hand sanitizer his hand . \textsc{<EOT>} \\

% \hline
%         \rowcolor{Gray}
%  \textsc{<BOT>} cleanliness is not on their radar . outside patio was filthy , server kept running his hand thru his hair . \\ \hline \hline
% \end{tabular}
%     }
%     \caption{
%     Interpolation results between latent code of input sentences from Yelp15 for sMIM (1024).
%     Input sentences $\x_i,\x_j$ are marked with gray, mid-sentences are decoded from interpolation 
%     between samples from the corresponding posteriors.
%     }
%     \label{tab:language-modelling-ptb-qualitative-interpolation-mim-1}
% \end{table}

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{0.5em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{p{8cm}}
%         \textbf{5 stars $\rightarrow$ 5 stars} \\ \hline \hline
%         \rowcolor{Gray}
% \textsc{<BOT>} very intimate restaurant . enjoyed the seven course meal with my wife . highly recommend for a memorable experience on mt . washington . \\
% \hline
% \textbullet ~ very intimate restaurant . highly recommend the meal with my wife enjoyed her experience . highly recommend for a memorable on a nice . experience . \textsc{<EOT>} \\
% \textbullet ~ very casual restaurant . love the fried pickles you are your . my wife enjoyed one with a good meal . i highly recommend it . \textsc{<EOT>} \\
% \textbullet ~ you love your fried pickles . i love the fried pickles . my one visit to pittsburgh are good . you are paying for your experience . \textsc{<EOT>} \\
% \textbullet ~ i love you fried pickles . i love your fried pickles . i are one to my good friend to visit  \textsc{<EOT>} \\
% \hline
%         \rowcolor{Gray}
%  \textsc{<BOT>} i love you penguin . i love your fried pickles . you are one good reason to visit my hometown . \\ \hline \hline
        \textbf{5 stars $\rightarrow$ 1 star} \\ \hline \hline
        \rowcolor{Gray}
\textsc{<BOT>} awesome food , just awesome ! top notch beer selection . great staff . beer garden is great setting . \\
\hline
\textbullet ~ awesome food , just top notch ! great beer selection . staff has great craft beer . top notch is that . \textsc{<EOT>} \\
\textbullet ~ awesome food ! just kidding , beer selection is great . staff has trained knowledge on top .  \textsc{<EOT>} \\
\textbullet ~ cleanliness is awesome ! not only on their game , food . server was polite his hand sanitizer outside .  \textsc{<EOT>} \\
\textbullet ~ cleanliness is not on their patio . server was outside , kept running his hand sanitizer his hand .  \textsc{<EOT>} \\
\hline
        \rowcolor{Gray}
 \textsc{<BOT>} cleanliness is not on their radar . outside patio was filthy , server kept running his hand thru his hair . \\ \hline \hline
\end{tabular}
    }
        \vspace*{-0.2cm}
    \caption{
    Interpolation results between latent codes of input sentences (with gray) from \textbf{Yelp15} for sMIM (1024).
    }
    \label{tab:language-modelling-ptb-qualitative-interpolation-mim-2}
    \vspace*{-0.15cm}
\end{table}


\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{0.5em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{l p{7cm} }
        \hline \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rowcolor{Gray}
(D) & \textsc{<BOT>} the company did n't break out its fourth-quarter results  \\
        \hline 
(M) & the company did n't break out its results \textsc{<EOT>} \\
(R) & the company did n't break out its fourth-quarter results \textsc{<EOT>} \\
(P) & the company did n't accurately out its results \textsc{<EOT>} \\
% (D) & \textsc{<BOT>} the \textsc{<UNK>} record of n million shares was set on oct . n \\
% (M) & the \textsc{<UNK>} of n million shares was shot on monday \textsc{<EOT>} \\
% (R) & the \textsc{<UNK>} purchase of n million shares was on oct . n \textsc{<EOT>} \\
% (P) & the \textsc{<UNK>} of n million shares was set on oct . n \textsc{<EOT>} \\
%         \hline \hline
%         \rowcolor{Gray}
%         \multicolumn{2}{l}{\textbf{sVAE (128)}} \\ \hline \hline

% (D) & \textsc{<BOT>} the \textsc{<UNK>} record of n million shares was set on oct . n \\
% (M) & under the new york stock exchange said peter \textsc{<UNK>} \textsc{<UNK>} a \textsc{<UNK>} partnership between ford ' s performance \textsc{<EOT>} \\
% (R) & a \textsc{<UNK>} of texas the underground \textsc{<UNK>} \textsc{<UNK>} textile \textsc{<UNK>} has led for loan defaults to \textsc{<UNK>} an interest-rate and gained a \textsc{<UNK>} from the council of its cleanup \textsc{<UNK>} where some a federal industrial state in a \textsc{<UNK>} they could end a substantial number of taxes and preparing a total \textsc{<EOT>} \\
% (P) & divergence erupted erupted adjustable adjustable adjustable adjustable adjustable adjustable ranges grip implies monte climate monte monte implies implies monte implies implies implies implies ... \\
    \end{tabular}
    }
    \vspace*{-0.2cm}
    \caption{
    % Reconstruction results for sMIM (512) and sVAE(128) models trained on PTB.
    Reconstruction results for sMIM (512) model trained on \textbf{PTB}.
    We denote:
    (D) Data sample; 
    (M) Mean (latent) reconstruction;
    (R) Reconstruction;
    (P) Perturbed (latent) reconstruction.
    % See text for details.
    % (D) Data sample $\x_i$, with a corresponding latent code sampled from the encoder
    % $\z_i \sim \Menc(\z | \x_i)$;
    % (M) Reconstruction $\x$ sampled conditioned on the mean of the posterior
    % $\hat{\x}_i \sim \Mdec(\x| \E{}{\z_i})$;
    % (R) Reconstruction $\x$ sampled conditioned on the latent code
    % $\hat{\x}_i \sim \Mdec(\x| \z_i)$;
    % (P) Reconstruction $\x$ sampled conditioned on the perturbed latent code
    % $\hat{\x}_i \sim \Mdec(\x| \z_i + \epsilon)$, where
    % $\epsilon \sim \mathcal{N}(\mu = 0, \sigma = 10 \sigma_{\z_i})$
    % is sampled from 10 times the variance of the corresponding encoder.
    }
    \label{tab:language-modelling-quantitative-ptb-recon}
    \vspace*{-0.2cm}
\end{table}

We further probe the structure in the learned representation, demonstrating that
sMIM learns a dense, meaningful latent space. We present latent interpolation results in
Table\ \ref{tab:language-modelling-ptb-qualitative-interpolation-mim-2}
for samples (\ie, reviews) with the different ratings from Yelp5. 
Interpolation entails sampling $\x \sim \Mdec(\x| \z_\alpha)$ where $\z_\alpha$ is interpolated at equispaced points  
between two randomly sampled latent codes, $\z_i \sim \Menc(\z|\x_i)$, and $\z_j \sim \Menc(\z|\x_j)$.

Next we show reconstruction, and perturbation
results for for sMIM (512) trained on PTB. 
Table\ \ref{tab:language-modelling-quantitative-ptb-recon} shows four sentences:
(D) the input sentence;
(M) the mean reconstruction given the posterior mean $z$;
(R) a reconstruction given a random sample $z$ from the posterior;
and 
(P) a {\em perturbed reconstruction}, given a sample $z$ from a Gaussian
distribution with 10 times the posterior standard deviation.
The high mutual information learned by sMIM leads to good reconstruction, as clear in (M) and (R).
sMIM also exhibits good clustering in the latent space, shown here by the similarity of (R) and (P).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Question-Answering} 
\label{sec:nlp-question-answering-yahoo}

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{0.2em} % for the horizontal padding
    {\footnotesize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular}{l||ccc}
        \hline
    Model & P@1 $\uparrow$ & MRR  $\uparrow$  \\
    \hline \hline
    AP-CNN \citep{DBLP:journals/corr/SantosTXZ16} & 0.560 & 0.726   \\
    AP-BiLSTM \citep{DBLP:journals/corr/SantosTXZ16} & 0.568 & 0.731  \\
    HyperQA \cite{DBLP:journals/corr/TayLH17a} &  \textbf{0.683} & 0.801   \\
    \hline
    sAE (32)  & 0.386 & 0.656 \\
    sAE (512)  & 0.579 & 0.814 \\
    sAE (1024)  & 0.519 & 0.767 \\
    \hline
    sVAE (32) + kl \textsuperscript{*} & 0.531 & 0.776 \\
    sVAE (512) + kl \textsuperscript{*} & 0.494 & 0.747 \\
    sVAE (1024) + kl \textsuperscript{*} & 0.548 & 0.79 \\
    \hline
    sMIM (32) \textsuperscript{\textdaggerdbl} & 0.558  & 0.737 \\
    sMIM (512) \textsuperscript{\textdaggerdbl} & \textbf{0.683} & \textbf{0.818} \\
    sMIM (1024) \textsuperscript{\textdaggerdbl} & 0.651 & 0.8 \\
    \hdashline[1pt/1pt]
    sAE (1024)  \textsuperscript{\textdagger} & 0.574 & 0.812 \\
    sVAE (1024) \textsuperscript{\textdagger}\textsuperscript{*} & 0.339  & 0.616 \\
    sMIM (1024) \textsuperscript{\textdagger} \textsuperscript{\textdaggerdbl} & \textbf{0.757} & \textbf{0.863} \\
        \hline
\end{tabular}
    }
        \vspace*{-0.1cm}
    \caption{
    {\bf YahooCQA} results for sMIM, AE, and single-task models.
    Results\textsuperscript{\textdaggerdbl} are averaged over 10 runs (stdev $< 0.002$).
    sMIM (1024)\textsuperscript{\textdagger} is pre-trained on Everything dataset. %PTB, Yahoo Answers, Yelp15 and WT103.
    sVAE\textsuperscript{*} results are based on the mean of the posterior, rather the sample \citep{bosc-vincent-2020-sequence}. 
    $P@1$ and MRR are defined in Sec.\ \ref{sec:nlp-question-answering-yahoo}.
    }
    \label{tab:question-answering-yahoocqa}
    \vspace*{-0.1cm}
\end{table}


% \textsc{<BOT>}

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{0.5em} % for the horizontal padding
    {\scriptsize
    \renewcommand{\arraystretch}{1.2}% for the vertical padding
        \begin{tabular}{p{8cm}}
         \hline
        \rowcolor{Gray}
Q: \textsc{<BOT>} my brother is geting out on parole from navy jail where can i find a parole office in our area \textsc{<UNK>} , \textsc{<UNK>} ? \\
\hline
A: you can find out the county jail , or call your local police station . \textsc{<EOT>} \\
\hline
%%%%%%%%%%%%%%%
         \hline
        \rowcolor{Gray}
Q: \textsc{<BOT>} what continent has most deserts ? \\
\hline
A: the most notable is in the netherlands . \textsc{<EOT>} \\
\hline
%%%%%%%%%%%%%%%
         \hline
        \rowcolor{Gray}
Q: \textsc{<BOT>} how do u clear the history in the search field ? \\
\hline
A:  u can find it in the search bar . \textsc{<EOT>} \\
\hline
%%%%%%%%%%%%%%%
         \hline
        \rowcolor{Gray}
Q: \textsc{<BOT>} what is the best question to ask ? \\
\hline
A: ask yourself ! \textsc{<EOT>} \\
\hline
%%%%%%%%%%%%%%%
         \hline
        \rowcolor{Gray}
Q: \textsc{<BOT>} need to find somewhere to sale baseball cards . ? \\
\hline
A: ebay \textsc{<EOT>} \\
\hline
%%%%%%%%%%%%%%%
         \hline
%         \rowcolor{Gray}
% Q: \textsc{<BOT>} what's the opposite of opposite ? \\
% \hline
% A: opposite opposite opposite ; i thought it really helps . \textsc{<EOT>} \\
% \hline
%%%%%%%%%%%%%%%
\end{tabular}
    }
        \vspace*{-0.1cm}
    \caption{
    Sampled answers from \textbf{Yahoo Answers} sMIM (1024).
    }
    \label{tab:question-answering-samples}
    \vspace*{-0.1cm}
\end{table}

So far we have discussed abstract aspects of representations learned by sMIM, such as high mutual information, and low marginal entropy.
To demonstrate the benefits of representations learned by sMIM, we consider a downstream task in which sMIM is 
pre-trained on Yahoo Answers, then used for question-answering on YahooCQA 
\citep{DBLP:conf/sigir/TayPLH17}, with no fine-tuning. 
% The YahooCQA vocabulary has 116,900 tokens, with training, validation and test sets
% having  253K, 31.7K and 31.7K QA pairs, respectively.
% These sets were constructed by taking a subset of the QA pairs from Yahoo Answers,
% from which each question is then paired with another 2-4 answers (not from Yahoo Answers).
% Thus each question, of 5-50 tokens, has 3-5 possible ranked answers  (1 is best).
% Let $Q_i$ denote the $i^{th}$ question, and let $ \{A_i^k\}_{k=1}^{K_i}$ be the $K_i$ 
% corresponding answers, ordered such that $A_i^k$ has rank $k$.
% To match the format of QA pairs in Yahoo Answers, we compose question-answer 
% pair  $Q_i^k$ by concatenating $Q_i$, "?", and $A_i^k$.
% % \footnote{As ranked by \url{http://lucene.apache.org/core/}}.
YahooCQA comprises questions and 3-5 answers, where the first answer is from Yahoo Answer, 
and the additional answers are wrong.
Let $Q_i$ denote the $i^{th}$ question, and let $ \{A_i^k\}_{k=1}^{K_i}$ be the $K_i$ 
corresponding answers, ordered such that $A_i^k$ has rank $k$.
To match the format of QA pairs in Yahoo Answers, we compose question-answer 
pair  $Q_i^k$ by concatenating $Q_i$, "?", and $A_i^k$.

For question-answering with sMIM we use the following procedure:
% Since sMIM was trained on sentences of the concatenated questions and answers  (\ie, $Q_i^1$),
For each question-answer we sample $\z_i^k \sim \Menc(\z|Q_i^k)$, and a corresponding 
$\z_i^{unk} \sim \Menc(\z|Q_i^{unk})$ where $Q_i^{unk}$ is simply $Q_i$ concatenated 
with "?" and a sequence of <unk> tokens to represent the $|A_i^k|$ unknown words of the answer.
% $( Q_i + \text{"?"} + \sum_{length(A_i^k)} \text{" <unk>"} )$,
We then rank question-answer pairs according to the score
$S_i^k = ||\z_i^{unk} - \z_i^k|| / \sigma_i^{k,unk}$
where $\sigma_i^{k,unk}$ is the standard deviation of $\Menc(\z|Q_i^{unk})$. 
In other words, we rank each question-answer pair according to the normalized distance between  
the latent code of the question with, and without, the answer. This score is similar 
to  $\log \Menc(\z_i^k|Q_i^{unk})$, but without taking the log standard deviation into account. 

As is common in the literature, Table\ \ref{tab:question-answering-yahoocqa} quantifies test performance 
using average precision 
($P@1 \!=\! \frac{1}{N} \sum_i\! \mathbbm{1}{(rank(A_i^1) = 1)}$), 
and Mean Reciprocal Ranking ($MRR = \frac{1}{N} \sum_i \frac{1}{rank(A_i^1)}$).
As baselines, we consider best performing single-task models trained directly on YahooCQA \citep{DBLP:journals/corr/SantosTXZ16,DBLP:journals/corr/TayLH17a}.
Interestingly, sMIM (512), pre-trained on Yahoo Answers, exhibits state-of-the-art 
performance compared to these baselines.
For an even larger sMIM model, pre-trained on all of PTB, Yahoo Answers, Yelp15
and WT103, the question-answering performance of sMIM is even better
(last row of Table\ \ref{tab:question-answering-yahoocqa}).

The results for sVAE are based on the mean of the posterior rather than a random sample.
This is a common heuristic in the NLP literature which has been proven useful for downstream tasks, 
but is problematic when considering the generative process which relies on the sample rather than the mean \citep{bosc-vincent-2020-sequence}. 
Finally, as another point of comparison, we repeated the experiment with a 
deterministic sAE model (with $\sigma_i^{k,unk} = 1$).
In this case performance drops, especially average precision, indicating that 
the latent representations are not as meaningfully structured.

Importantly, sMIM can generate novel answers rather than simply ranking a given set of alternatives.
To this end, we sample $\z_i^{unk} \sim \Menc(\z_i^k|Q_i^{unk})$, as described above,
followed by modified reconstruction $\widehat{Q}_i \sim \Mdec(\x|\z_i^{unk})$. 
We modify the sampling procedure to be greedy (\ie, top 1 token), and prevent 
the model from sampling the "\textsc{<UNK>}" token.
We consider all words past the first "?" as the answer. (We also removed HTML tags (\eg, "<br>").)
Table\ \ref{tab:question-answering-samples} gives several selected answers.
The examples were chosen to be short, and with appropriate (non-offensive) content.
We note that we did not use any common techniques to manipulate the decoding distribution,
such as beam search, Nucleus sampling \citep{DBLP:journals/corr/abs-1904-09751}, or sampling with temperature \citep{ACKLEY1985147}.
To the best of our knowledge, sMIM is the current state-o-the-art for a {\em single-task} model for YahooCQA, 
despite having simpler architecture and training procedure when compared to competing models.

% \micha{I couldn't find better results for YahooCQA. There might exist some better papers, but I am not sure if we want to address that. Thoughts?}\kevin{If you've given a thorough lit review, then I would say ``to the best of our knowledge''. This is a hedge against missing something. Part of the reviewer's job is to point out missing references.}
% We also acknowledge that recent work get better results in multi-task settings, whereas here we are concerned with a zero-shot settings (\ie, a single task).


==> 2021-04-21 - SentenceMIM/sections/formulation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Problem Formulation}

Let $\x \in \mathcal{X} = \{\x_i\}_{i=1}^{X}$ be a discrete variable representing
a sequence of $T$ tokens from a finite vocabulary $\mathcal{V}$.
A sequence might be a sentence or a paragraph, for example.
% , or any other text excerpt which holds a semantic meaning (\eg, a question and answer).
The set $\mathcal{X}$ comprises all sequences we aim to model.
The size of $\mathcal{X}$, \ie, $X$, is typically unknown and large.
Let $\pjoint(\x)$ be the unknown probability of sentence $\x \in \mathcal{X}$.

We model the distribution over a sequence of length $T$ as an auto-regressive distribution over $T+1$ tokens, 
where the additional end-of-text special token\footnote{\textsc{<BOT>}, \textsc{<EOT>} are a special beginning/end-of-text tokens. The token \textsc{<UNK>} represents an out-of-vocabulary word.},  \textsc{<EOT>}, 
% models the probability of the sequence being of length $T$. 
effectively captures the probability that the sequence length is $T$.
More explicitly, we model the following distribution
\begin{equation}
    \pjoint(\x) = \prod_{k=0}^{T} \pdec(x^k | \x^{<k})
\end{equation}
where $\x^{<k}$ denotes the tokens preceding $x^k$,
$\pdec(x^k | \x^{<k})$ is a categorical distribution over $\mathcal{V}$, 
and $\pdec(x^{T} = \text{\textsc{<EOT>}} | \x^{<T})$ is the probability that $T$ is the sentence length.

We learn a latent variable model given $N$ fair samples from $\pjoint(\x)$, where $N \ll X$, with
discrete observations $\x \in \mathcal{X}$, and a continuous latent space $\z \in \mathbb{R}^{d}$.
The encoder, $\Menc(\z | \x)$, maps sequences to a distribution over continuous latent codes,
and a corresponding decoder, $\Mdec(\x|\z)$, maps a latent code to a distribution over sequences.
Let $\params$ be the joint parameters of the encoder and decoder.

% Ideally the encoder maps inputs to latent codes from which
% the decoder can correctly reconstruct the input.
% We also desire a latent space in which similar sentences
% (\eg, in structure or content) are mapped to nearby latent codes.

% To that end, we would like to learn a model with a high mutual information, and low marginal entropy.
% High mutual information will encourage an approximately deterministic mapping (\ie, good reconstruction).
% Low marginal entropy will encourage better compression scheme,
% which hopefully leads to a semantic clustered representation.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Encoder-Decoder Specification} \label{sec:nlp-formulation}

\begin{figure}[t]
    \centering
    \scalebox{0.85}{\input{diag/model-arch-decoder}}
    % \includegraphics[width=0.8\columnwidth]{images/diag/decoder.pdf}
    \vspace*{-0.6cm}
    \caption{The decoder, implemented with GRU, is auto-regressive and conditioned on latent code $\z$.
    Words are represented by parametric embeddings.
    At each step the inputs are the latent code and previous output token.
    The GRU output provides a categorical distribution over tokens $\x^k$,    %  \in \mathcal{V}$, 
    from which the next token is sampled.
    % The top sentence depicts the sample, with inputs on the bottom.
    % <BOT>/<EOT> are the start/end-of-sentence tokens.
    }
    \label{fig:sentence-mim-arch-decoder}
\end{figure}


In what follows we adapt the architecture proposed by \citet{DBLP:journals/corr/BowmanVVDJB15}, 
the main difference being the use of GRUs \citep{cho-etal-2014-learning} instead of LSTMs \citep{Hochreiter:1997:LSM:1246443.1246450}.
We opt for a simple architecture instead of more recent variants, such as Transformers \citep{Vaswani2017}
or AWD-LSTMs \citep{merity2018regularizing}, to focus on the effect of the learning framework on a given architecture (\ie, MIM, VAE, AE), 
rather than the architecture itself.

Beginning with the generative process, let $\Mdec(\x|\z) $ be a conditional auto-regressive distribution 
over a sequence of $T$ tokens, $\x = (x^{0},\ldots, x^{T-1}, x^{T} = \text{\textsc{<EOT>}})$,
% with tokens $x^k \in \mathcal{V}$, as
% \begin{eqnarray}
%     \log \Mdec(\x|\z) \!\! &=& \!\! \log \Mdec(x^1|\z) \\
%     && \! + ~ \sum_{k=2}^{T} \log \Mdec(x^k\, |\, x^{k-1},\ldots, x^1, \z) \nonumber
%     \label{eq:p-x-seq-given-z}
% \end{eqnarray}
\begin{equation}
    \log \Mdec(\x|\z) \, =\, \sum_{k=0}^{T} \log \Mdec(x^k\, |\, \x^{<k}, \z)
    \label{eq:p-x-seq-given-z}
\end{equation}
where $\Mdec(x^k | \cdot )$ is a categorical distribution over $|\mathcal{V}|$
possible tokens for the $k^{th}$ element in $\x$.
According to the model (Fig.\ \ref{fig:sentence-mim-arch-decoder}), generating
a sentence $\x$ with latent code $\z$ entails sampling each token from a
distribution conditioned on the latent code and previously sampled tokens.
Tokens are modelled with a parametric embedding. Conditioning the distribution over $\z$
entails concatenating $\z$ to the input embeddings per token \citep{DBLP:journals/corr/BowmanVVDJB15}.

\begin{figure}[t]
    \vspace*{-0.01cm}
    \centering
    \scalebox{0.85}{\input{diag/model-arch-encoder}}
    % \includegraphics[width=0.6\columnwidth]{images/diag/encoder.pdf}
     \vspace*{-0.6cm}
    \caption{The encoder is implemented with GRU.
    Each word is represented by a parametric embedding.
    Given the input sequence, the encoder maps the last hidden state % (\ie, depends on all the tokens) 
    to the mean and variance of a Gaussian posterior over latent codes.
    % <BOT> is the start-of-sentence token.
    }
    \label{fig:sentence-mim-arch-encoder}
    \vspace*{-0.1cm}
\end{figure}


The encoder $\Menc(\z|\x)$ is the posterior distribution over the latent variable $\z$,
conditioned on a sequence $\x$.  We take this to be Gaussian whose mean and diagonal 
covariance are specified by mappings $\mu_\params$ and  $\sigma_\params$:
\begin{equation}
    \Menc(\z|\x) \, =\, \mathcal{N}(\z; \mu_\params(\x), \sigma_\params(\x))
    \label{eq:nlp-q-z-given-x}
\end{equation}
Linear mappings $\mu_\params$ and  $\sigma_\params$ are computed from the last hidden state of a GRU (see Fig.\ \ref{fig:sentence-mim-arch-encoder}).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{MIM Learning Objective}
\label{sec:nlp-learning}

The Mutual Information Machine (MIM) \cite{2019arXiv191003175L} is a versatile generative LVM 
which can be used for representation learning, and sample generation.
% probability density estimation, 
MIM learns a model with high mutual information between observations and latent codes,
and is robust against posterior collapse. % with language data.
% (cf., \citet{DBLP:journals/corr/BowmanVVDJB15, bosc-vincent-2020-sequence}).

The MIM framework begins with two {\em anchor} distributions, $\pjoint(x)$ and $\pjoint(z)$, for
observations and the latent space, from which one can draw samples.  They are fixed and not learned.
MIM also has a parameterized encoder-decoder pair, $\Menc(\z|\x)$ and $\Mdec(\x|\z)$,
and parametric marginal distributions $\Menc(\x)$ and $\Mdec(\z)$.
These parametric elements define joint encoding and decoding {\em model} distributions:
\begin{eqnarray}
    \Menc(\x,\z) & = & \Menc(\z|\x)~ \Menc(\x) ~, \\
    \Mdec(\x,\z) & = & \Mdec(\x|\z)~\Mdec(\z) ~ .
\end{eqnarray}
MIM learning entails the minimization of the cross-entropy between a sample distribution 
and the model encoding and decoding distributions \citep{2019arXiv191003175L}. 
This simple loss constitutes a variational upper bound on a regularized Jensen-Shannon divergence, 
resembling VAE in which a model distribution matches samples from a sample distribution via KL 
divergence minimization \citep{Zhao_Song_Ermon_2018}. 
Fundamentally, MIM learning differs from VAE learning, with the former being an upper bound on the 
joint cross-entropy, while the latter being an upper bound on the marginal cross-entropy of the observations.

MIM requires sampling from the decoder during training, which can be slow for sequential computational models.
For language modeling we therefore use A-MIM learning, a MIM variant that minimizes a loss
defined on the encoding and decoding distributions, with samples drawn from an encoding 
{\em sample} distribution, denoted  $\Msamp^{\penc}(\x, \z)$;  \ie,
\begin{eqnarray}
    \Msamp^{\penc}(\x, \z) ~=~ \Penc \label{eq:sample-dist} ~.
\end{eqnarray}
The A-MIM loss is defined as follows,
\begin{eqnarray}
    \AMIMloss(\params) &=&
    \frac{1}{2} \big(\, \CE{\Msamp^{\penc}(\x, \z)}{\Menc \left(\x, \z \right)} \label{eq:A-MIM-asymmetric-bound} \\
    && \quad + ~ \CE{\Msamp^{\penc}(\x, \z)}{\Mdec \left(\x, \z \right)} \, \big) \nonumber \\
    &\geq& H_{\Msamp^{\penc}} (\x) + H_{\Msamp^{\penc}} (\z)  - I_{\Msamp^{\penc}} (\x;\z)~,
    \nonumber
\end{eqnarray}
where $\CE{\cdot}{\cdot}$ is cross-entropy, $H_{\Msamp^{\penc}}(\cdot)$ is information entropy over
distribution $\Msamp^{\penc}$, and $I(\cdot;\cdot)$ is mutual information.
Minimizing $\AMIMloss(\params)$ learns a model with a consistent
encoder-decoder, high mutual information, and low marginal entropy \citep{2019arXiv191003175L}.
The A-MIM loss is in fact a variational upper bound on the joint entropy of the encoding 
sample distribution.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Implicit and Explicit Model Marginals} \label{sec:nlp-variational-priors}

To complete the model specification, we define the model marginals $\Menc(\x)$ and $\Mdec(\z)$.
We call the marginal {\it explicit}  when we can evaluate the probability of a sample 
under the corresponding distribution, and {\it implicit} otherwise.

Examples of explicit marginals are a Gaussian for $\Mdec(\z)$, and an auto-regressive distribution for $\Menc(\x)$. 
They enable evaluation of the probability of a sample straightforwardly. 
% An explicit distribution allows us to introduce inductive bias in the model. For example, a Gaussian distribution 
% for $\Mdec(\z)$ assumes smoothness in the probability density, and isomorphy in the latent dimensions.
However, the inductive bias in such distributions, or the architecture, can lead to a  challenging optimization problem. 
% In practice, introducing an explicit distribution often lead to worse optimum in the model.

An implicit marginal distribution can be defined via marginalization of a joint distribution.  
To help encourage consistency, and avoid introducing more model parameters, one can
define model marginals in terms of the sample distributions, like $\Msamp^{\penc}(\x, \z)$ above \citep{DBLP:journals/corr/BornscheinSFB15,2019arXiv191003175L,DBLP:journals/corr/TomczakW17}.
They allow one to share parameters between a marginal and the corresponding conditional distribution, 
and to reduce the inductive bias in the architecture. 
Unfortunately, evaluating the probability of a sample under an implicit distribution is intractable in general.

We define $\Menc(\x)$ as a marginal over the decoder \cite{DBLP:journals/corr/BornscheinSFB15}; \ie,
\begin{equation}
     \Menc(\x) \, = \, \E{\pjoint(\z)}{\Mdec(\x|\z)}  ~,
    \label{eq:nlp-q-x}
\end{equation}
where the latent anchor is defined to be a standard normal, $\pjoint(\z) = \mathcal{N}(\z ; 0, 1)$.
Similarly, the model density over latent codes is defined as
\begin{equation}
    \Mdec(\z) \,=\,  \E{\pjoint(\x)}{\Menc(\z|\x)}~.
    \label{eq:nlp-p-z}
\end{equation}
\ie, the latent marginal is defined as the aggregated posterior, in the spirit of the 
VampPrior \cite{DBLP:journals/corr/TomczakW17} and Exemplar VAE \cite{ExemplarVAE2020}.




\subsection{Tractable Bounds to Loss}

Given training data $D = \{\x_i \}_{i=1}^N$, the empirical loss is
\begin{eqnarray}
    \!\EAMIMloss (\params) \!\!\!\!
    &=& \!\!\!
    - \frac{1}{2N}
    \sum_{\x_i}\! \E{\Menc(\z|\x_i)}{\log  \Menc(\z|\x_i)\,\Menc(\x_i)} \nonumber \\
    && \hspace*{-0.65cm}
    - ~ \frac{1}{2N}
    \sum_{\x_i}\! \E{\Menc(\z|\x_i)}{\log \Mdec(\x_i|\z)\,\Mdec(\z)} ~
    \label{eq:nlp-mim-loss-empirical}
\end{eqnarray}
where $\sum_{\x_i}$ denotes a sum over $N$ fair samples drawn from $\pjoint(\x)$, 
as a MC approximation to expectation over $\pjoint(\x)$.

Unfortunately, the empirical loss in Eqn.\ \eqref{eq:nlp-mim-loss-empirical} is intractable since we
cannot evaluate the log-probability of the marginals $\Mdec(\z)$ and $\Menc(\x)$.
In what follows we obtain a tractable empirical bound on the loss in Eqn.\ \eqref{eq:nlp-mim-loss-empirical}
for which, with one joint sample, we obtain an unbiased and low-variance estimate of the gradient using reparameterization \cite{Kingma2013}.

We first derive a tractable lower bound to $\log \Menc(\x_i)\, $:
\begin{eqnarray}
    \log \Menc(\x_i)\!\! &\underset{\text{\tiny (Eqn. \ref{eq:nlp-q-x})}}{=}& \!\log \E{\pjoint(\z)}{\Mdec(\x_i|\z)}  \label{eq:nlp-q-x-lower-bound} \\
    &\underset{\text{\tiny (IS)}}{=}& \!\log \E{\Menc(\z|\x_i)}{\Mdec(\x_i|\z)\frac{\pjoint(\z)}{\Menc(\z|\x_i)}}
     \nonumber \\
    &\underset{\text{\tiny (JI)}}{\ge}& \!\E{\Menc(\z|\x_i)}{\log \left(  \Mdec(\x_i|\z)\frac{\pjoint(\z)}{\Menc(\z|\x_i)} \right) }  \nonumber
\end{eqnarray}
where the second and third lines are obtained using importance sampling and Jensen's inequality.
We remind the reader that $\Menc(\x_i)$ is a variational marginal that can depend
on $\x_i$.  Indeed, Eqn.\ \eqref{eq:nlp-q-x-lower-bound} is the usual ELBO.

To derive a lower bound to $\log \Mdec(\z)$, we begin with the following inequality,
\begin{eqnarray}
\!\!\log \E{\pjoint(\x)}{h(\x;\cdot)}  \!\!
&=& \!\!  \log \sum_{i} \pjoint(\x_i)\, h(\x_i;\cdot) \nonumber  \\
&\ge& \!\log \pjoint(\x')\, h(\x';\cdot) ~,
\label{eq:log-lower-bound}
\end{eqnarray}
for any sample $\x'$, any discrete distribution $\pjoint(\x)$, and any non-negative function $h(\x;\cdot) \ge 0$.
The inequality in Eqn.\ \eqref{eq:log-lower-bound} follows from $\log a \ge \log b$ for $a \ge b$.
Using this bound, we express a lower bound to $\Mdec(\z)$ as follows,
\begin{eqnarray}
    \log \Mdec(\z) &\underset{\text{\tiny (Eqn. \ref{eq:nlp-p-z})}}{=}& \log \E{\pjoint(\x)}{\Menc(\z|\x)} \nonumber \\
    &\underset{\text{\tiny (Eqn. \ref{eq:log-lower-bound})}}{\ge}& \log \Menc(\z|\x')  + \log \pjoint(\x') \label{eq:nlp-p-z-lower-bound}
\end{eqnarray}
for any sample $\x'$. During training, given a joint sample $~\x_i, \z_i \sim \Penc$, we choose $\x' = \x_i$.

\begin{figure}[t]
\vspace*{-0.35cm}
\centering
\begin{minipage}[t]{0.95\columnwidth}
\begin{algorithm}[H]
    \caption{Learning parameters $\params$ of sentenceMIM}
    \label{algo:sentencemim}
    \begin{algorithmic}[1]
        % \REQUIRE Samples from anchors $\pjoint(\x)$
        \WHILE{not converged}
        \STATE $D_\mathrm{enc} \gets \{ \x_j, \z_j \sim \Menc(\z|\x)\pjoint(\x) \}_{j=1}^{N}$
        \STATE $\EMIMloss \left( \params ; D \right) = -\frac{1}{N}\! \sum_{i=1}^{N}\! \big( ~ \log \Mdec(\x_i | \z_i) ~~~~~~
        \linebreak ~~~~~~~~~~~~~~~~~~  + \frac{1}{2} \left( \log \Menc(\z_i | \x_i) + \log \pjoint(\z_i) \right) ~ \big)$
        \STATE $\Delta \params \propto -\nabla_{\params}  \EMIMloss \left( \params ; D \right)$
        \COMMENT{\textcolor{gray}{\textit{Gradient computed through sampling using reparameterization}}}
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace*{-0.5cm}
\end{figure}


Substituting Eqns.\ \eqref{eq:nlp-q-x-lower-bound} and \eqref{eq:nlp-p-z-lower-bound}
into Eqn.\ \eqref{eq:nlp-mim-loss-empirical} gives the final form of an
upper bound on the empirical loss; \ie,
\begin{eqnarray}
    \EAMIMloss \!\!
    & \le & \!\! -\frac{1}{N} \, \sum_{i} \E{\Menc(\z |\x_i)}{\log \Mdec(\x_i|\z)}  \nonumber \\
    & & -\frac{1}{2N} \, \sum_{i} \E{\Menc(\z |\x_i)}{\log \big( ~ \Menc(\z|\x_i) \pjoint(\z) ~ \big) } \nonumber \\
    & & + \frac{1}{2}\HD{\pjoint}{\x} ~. \label{eq:nlp-mim-loss-empirical-bound}
\end{eqnarray}
We find an unbiased, low variance estimate of the gradient of Eqn.\ \eqref{eq:nlp-mim-loss-empirical-bound}
with a single joint sample $\z_i, \x_i \sim \Penc$ and reparameterization.
The last term, $\HD{\pjoint}{\x}$, is a constant, independent of model parameters
and can therefore be ignored during optimization.
The resulting learning process is described in Algorithm\ \ref{algo:sentencemim}.

To better understand the proposed bounds, we note that A-MIM achieves good
reconstruction by learning posteriors with relatively small variances
(\ie, relative to the distance between latent means).
Our choice of $\x'=\x_i$ exploits this, allowing good gradient estimation,
and facilitating fast convergence.
We further provide empirical evidence for these properties below in Fig.\ \ref{fig:nlp-dist-ptb}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Evaluating Implicit Prior Over Observations} \label{sec:nlp-evaluation}

% Defining the prior $\Menc(\x)$ to be the expectation over the decoder $\Mdec(\x|\z)$ can be viewed
% as a parameter-sharing scheme, which allows us to define the marginal without explicitly
% training a powerful probability density estimator, and without introducing architecture-related inductive bias.

% As an alternative, we can construct an explicit marginal over $\mathcal{X}$ with an implicit marginal using the procedure below,
% \begin{eqnarray}
%     \Menc(\x_n | \x_{i<n} ) &=&  \Mdec(\x | \z = \z')  \label{eq:nlp-q-x-explicit} \\
%     \z' & = & \E{z}{\Menc(\z | \x_{i<n} )}
% \end{eqnarray}
% where we repeat the procedure $T$ times for a sequence of length $T$.
% We note that using the same procedure during training is not a practical solution, due to excessive memory requirements, following the multiple passes of the encoder.
% The advantage of Eq.\ \eqref{eq:nlp-q-x-explicit} is that we can now evaluate the PPL over a held-out corpus directly, without the need to resort to approximation (\ie, using ELBO).
% Interestingly, Eq.\ \eqref{eq:nlp-q-x-explicit} can viewed as a PPL  downstream task.
% \micha{Show that sampling with random z for VAE results in similar PPL}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{NLL Evaluation} \label{sec:nlp-evaluation}

% As an alternative to the ELBO bound on log likelihood, here we propose
% an new bound that is better suited to models with implicit priors.
% With implicit priors, both NLL and ELBO are computationally expensive to estimate.
% Unlike ELBO, the new bound, called \MELBO (for MIM-ELBO) does not entail the evaluation
% of the log-likelihood of the latent model marginal.
% In the VAE literature, it is common to change the prior once the encoder and decoder
% have been trained (\eg, \citet{DBLP:journals/corr/abs-1901-03416, van2017neural}).
% Interestingly, if post-hoc we change the latent prior to be a marginal distribution,
% as in Eqn.~\ref{eq:nlp-p-z}, then \MELBO can be used to bound the NLL.
% This is particularly effective when the aggregated posterior is a poor fit to
% the original Gaussian prior, which is penalized heavily in the EBLO.

% Here we discuss model evaluation under a given empirical target distribution $\mathcal{T}(\x)$,
% and in particular, the empirical test set.
% We start with a bound on $\log \Mdec(\x_i)$, \ie,
% \begin{eqnarray}
%  \! \log \Mdec(\x_i) && \hspace*{-0.6cm} =~ \log \E{\Mdec(\z)}{\Mdec(\x_i|\z)} \nonumber \\
%     && \hspace*{-1.35cm}
%     \underset{\text{\tiny (IS)}}{=}~ \log \E{\Menc(\z|\x_i)}{\Mdec(\x_i|\z) \frac{\Mdec(\z)}{\Menc(\z|\x_i)} }
%     \nonumber \\
%     && \hspace*{-1.35cm}
%     \underset{\text{\tiny (Eqn. \ref{eq:nlp-p-z})}}{=} \, \log \E{\x' \sim \mathcal{T}(\x),\Menc(\z|\x_i)}{\Mdec(\x_i|\z) \frac{\Menc(\z|\x')}{\Menc(\z|\x_i)} }
%     \nonumber \\
%     && \hspace*{-1.35cm}
%     \underset{\text{\tiny (Eqn. \ref{eq:log-lower-bound})}}{\ge} \, \log \E{\Menc(\z|\x_i)}{\Mdec(\x_i|\z)}  + \log \mathcal{T}(\x_i)
%     \label{eq:log-lower-bound-p-x}
% \end{eqnarray}
% where the second step uses importance sampling,
% and the variational marginal in Eqn.\ \eqref{eq:nlp-p-z} is defined here under
% the target empirical distribution $\mathcal{T}(\x)$ in the last step.
% This allows us to choose $\x' = \x_i$, motivated by the tendency for MIM to learn
% highly clustered representations (cf.\ Fig.\ \ref{fig:nlp-dist-ptb}).
% We can also view Eqn.\ \eqref{eq:log-lower-bound-p-x} as an alternative
% to the usual ELBO; we refer to it as {\em \MELBO} (\ie, MIM ELBO).
% Like the ELBO, this bound holds for each data point, independent of target distribution $\mathcal{T}(\x)$.

% We can now derive an upper bound on the NLL under $\mathcal{T}$ using the \MELBO:
% \begin{eqnarray}
%     & & \mkern-46mu \hspace*{-0.4cm}  - \E{\mathcal{T}(\x)}{\log \Mdec(\x) } \label{eq:nll-upper-bound} \\
%     &\underset{\text{\tiny (Eqn. \ref{eq:log-lower-bound-p-x})}}{\le}& - \E{\Menc(\z|\x)\mathcal{T}(\x)}{\log \Mdec(\x|\z) } + H_\mathcal{T}(\x) \nonumber \\
%     & \underset{\text{\tiny (MC)}}{\lessapprox} & - \frac{1}{N} \, \sum_{\x_i} \left( \frac{1}{N_\z} \sum_{j=1}^{N_\z} \log \Mdec(\x_i|\z_{i,j}) \right) + \log N  \nonumber
% \end{eqnarray}
% where $\x_i \in D$, and $N_\z$ samples $\z_{i,j}$ are drawn from the encoder $\Menc(\z|\x_i)$.
% The last inequality follows $\log N$ being an upper bound on the entropy for the empirical distribution $\mathcal{T}(\x)$.
% We denote this empirical upper-bound by $\widehat{NLL}$,
% and the corresponding perplexity (PPL) upper bound by
% $\widehat{PPL} \equiv \exp(\frac{N \cdot \widehat{NLL}}{\sum_i T_i}) \ge PPL$,
% where $\sum_i T_i$ is the total number of tokens in a dataset with N samples.

% For the sizes of the datasets we consider, \MELBO and ELBO
% tend to be comparable for VAE.
% Notice that $\widehat{NLL}$ grows with the number of unique sentences  in the dataset
% (\ie, categories of a discrete variable), as expected from a categorical distribution.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Implicit Marginals} \label{sec:nlp-implicit-marginals}

% The motivation for constructing an expressive prior around the variational posterior
% is rooted in \emph{posterior holes} in VAE (coined by \cite{Rezende2018TamingV}).
% The term refers to the observation that the aggregated posterior in VAE assigns only
% a small probability mass to some areas of high probability under the prior.
% \cite{DBLP:journals/corr/TomczakW17} address the problem by learning the prior as a mixture model of the
% posterior with learnable pseudo-inputs (VampPrior).
% We point that VampPrior is a parametric approximation of
% Eqn.\ \eqref{eq:nlp-p-z-marginal} by means of learnable pseudo-inputs.
% Here we follow a similar path, and explicitly define the prior to match the aggregated posterior.
% As a side note, we mention that replacing VampPrior with Eqn.\ \eqref{eq:nlp-p-z-marginal}
% in VAE learning leads to severe collapse, and various regularization techniques
% are required to mitigate it. This research direction is out of the scope of this thesis,
% and we leave it for future research.

% To better understand the implications of implicit marginals, we point the reader to \cite{pmlr-v80-kim18e},
% which introduce Semi-Amortized VAE (SA-VAE). \cite{pmlr-v80-kim18e} propose to initialize a stochastic
% variational inference (SVI, \cite{JMLR:v14:hoffman13a}) with
% the output of an amortized recognition network. The resulting model learns a per-instance
% variational posterior (\ie, implicit priors here) which maximizes the ELBO for a particular observation.

% Interestingly, we find the inference network in MIM to produces a near optimal SVI (\ie, per-instance) solution,
% without the need for further per-instance optimization, characterized with low variance posterior and good reconstruction.
% This was also suggested by \cite{Hornik:1989:MFN:70405.70408}, when a rich-enough inference network is used.
% This is in contrast to \cite{pmlr-v80-kim18e} which report meaningful gains by SA-VAE (\ie, compared to VAE).
% We emphasize here that this is an empirical observation and further exploration is needed
% to establish the near-optimality of MIM amortized inference.

% We hypothesize that posterior collapse in VAE with Amortized VI (AVI) is the culprit
% for the need for further optimization to get good per-instance variational inference,
% and that the lack of such a collapse
% in amortized MIM learning leads to a near optimal AVI results. We leave that question open for future research.
% We demonstrate in Section\ \ref{sec:nlp-experiments} that despite the lack of a tractable prior, $\Mmodel$ offers superior NLL over the
% observations (\ie, when compared to $\Mmodel$), equal or better semantic latent interpolation,
% and superior sampling.


==> 2021-04-21 - SentenceMIM/sections/introduction.tex <==
\section{Introduction}

Generative modelling of text has become one of the predominant approaches to natural language processing (NLP), particularly in the machine learning community. 
It is favoured because it supports probabilistic reasoning and it provides a principled framework for unsupervised learning in the form of maximum likelihood. 
Unlike computer vision, where various generative approaches have proliferated~\cite{dinh2016density,goodfellow2014generative,Kingma2013,oord2016pixel,Rezende2014,vahdat2020NVAE}, 
current methods for text mainly rely on auto-regressive models (\eg, \citet{brown2020language}).

Generative latent variable models (LVMs), such as the variational auto-encoder 
(VAE) \cite{Kingma2013,Rezende2014}, are versatile and have been 
successfully applied to myriad domains.  
Such models consist of an encoder, which maps observations to distributions over 
latent codes, and a decoder that maps latent codes to distributions over observations.
LVMs are widely used and studied because they can learn a latent 
representation that carries many useful properties. 
Observations are encoded as fixed-length vectors that capture salient information, 
allowing for semantic comparison, interpolation, and search.
They are often useful in support of downstream tasks, such as transfer or k-shot learning. 
They are also often interpretable, capturing distinct factors of variation in different latent dimensions.
These properties have made LVMs especially compelling in the vision community.

Despite their desirable qualities, generative LVMs have not 
enjoyed the same level of success with text data. 
There have been recent proposals to adapt VAEs to text~\cite{DBLP:journals/corr/BowmanVVDJB15,  Guu2017GeneratingSB, KruengkraiACL2019,LiEtAlICNLG2019, DBLP:journals/corr/YangHSB17,bosc-vincent-2020-sequence}, 
but despite encouraging progress, they have not reached the same level of performance on natural 
language benchmarks as auto-regressive models
(\eg, \citep{DBLP:journals/corr/abs-1708-02182,DBLP:journals/corr/abs-1803-10049,pmlr-v97-wang19f}).
This is often attributed to the phenomenon of posterior collapse \citep{Fang_iLVM_2019_EMNLP,Li2019ASV},
in which the decoder captures all of the modelling power and the encoder conveys little to no information. 
For text, where the decoder is naturally auto-regressive, this has proven challenging to mitigate. 
A notable exception by \citet{li2020_Optimus} utilizes pre-trained BERT encoder
\citep{devlin-etal-2019-bert} and GPT-2 decoder \citep{Radford2019LanguageMA} in order to train a powerful VAE model. 
While showing strong PPL results, the training requires carefully designed heuristics to reduce posterior collapse.

This paper introduces sentenceMIM (sMIM), a new LVM for text. We use the Mutual Information Machine (MIM) framework 
by \citet{2019arXiv191003175L} for learning, and base our architecture on \citet{DBLP:journals/corr/BowmanVVDJB15}.
MIM is a recently introduced LVM framework that shares the same underlying architecture 
as VAEs, but uses a different learning objective that is robust against posterior collapse. 
MIM learns a highly informative and compressed latent representation, and often strictly 
benefits from more powerful architectures. 

% \micha{I added a lot of the text below}
We argue that an ideal LVM should be able to capture all aspects of variation of variable-size text observations 
within a fixed-size latent representation.
As such, high-dimensional latent codes are required, which is challenging with VAEs.
An ideal  model should provide excellent reconstruction, with fixed-size codes for variable-length sentences,
and be useful for various downstream tasks.

Auto-encoders (AEs)  \cite{NIPS1993_9e3cfc48} provide excellent reconstruction, 
but lack useful semantic structure in the learned representations.
AEs also allow one to learn high dimensional latent codes, only limited in practice by over-fitting.
VAEs, on the other hand, encourage semantic representations by regularizing the distribution over latent codes to match a given prior.
% (\ie, typically a Gaussian).
Such regularization, however, also contributes to posterior collapse, limiting the dimension of latent codes and reconstruction quality.
Here we propose MIM learning to enable high dimensional representations, while encouraging low latent entropy (under certain conditions) to promote clustering of semantically similar observations.
By encouraging the latent codes to match a known distribution we preserve the ability generate samples.
The resulting model offers a learned representation with high mutual information (\ie, to capture aspects of 
variation in the data), with low marginal entropy (\ie, introducing semantic structure to the learned representation), 
while aligning the latent distribution with a known prior.
sMIM also requires no hyper-parameter tuning for the loss, similar to AEs, which simplifies training.

This paper explores and contrasts properties of VAE learning, MIM learning, and AE learning on four well-known
text datasets, all with similar architectures.
We show that sMIM provides better reconstruction than VAE models, matching the reconstruction accuracy of AEs,
but with semantically meaningful representations, comparable to VAEs.
We further demonstrate the quality of the sMIM representation by generating diverse 
samples around a given sentence and interpolating between sentences. 
Finally, we show the versatility of the learned representation by applying a pre-trained sMIM 
model to a question answering task with state-of-art performance as compared to single task, supervised models.



==> 2021-04-21 - SentenceMIM/sections/intronotes.tex <==
Generative modelling of text has become one of the predominant approaches to natural language processing (NLP), particularly in the machine learning community. It is favoured because it allows for probabilistic reasoning, provides a principled learning framework (maximum likelihood). Unlike computer vision, where a variety of generative approaches have proliferated [], current methods for text mainly rely on auto-regressive models.

As an alternative, the family of generative latent variable models (LVMs), particularly variational auto-encoders (VAEs) [], have been successfully applied to many other domains. LVMs are widely studied because they can generate a latent representation that carries many useful properties. These are encoded as fixed-length vectors that capture salient semantic information, allowing for semantic comparison, interpolation, and search. They are often more interpretable, capturing distinct factors of variation in different latent dimensions. These properties have made LVMs especially compelling in the vision community [].

Despite their desirable qualities, LVMs have not enjoyed the same level of success in text modelling. There have been several proposals in recent years to adapt VAEs to text [], however these have not reached the same level of performance on natural language benchmarks as auto-regressive approaches. This is mainly attributed to the phenomenon of posterior collapse. A VAE consists of an encoder that maps data to a latent representation, and a decoder that maps the latent representation to data. In the case of posterior collapse, the decoder captures all of the modelling power and the encoder ends up conveying little to no information. For text, where the decoder itself is typically auto-regressive, this has proven challenging to mitigate.

In this paper, we introduce a new LVM for text based on the mutual information machine (MIM) framework [] called SentenceMIM. MIM is a recently introduced LVM framework that shares the same underlying architecture as a VAE, but uses a different learning objective that is more robust against posterior collapse. MIM learns a highly informative and compressed latent representation and often strictly benefits from more powerful architectures. VAE evaluation involves estimating a lower bound on the model log-likelihood called the evidence lower bound, or ELBO. Here, we propose an novel bound on the model log-likelihood for evaluating MIM models.

We show on four challenging datasets that SentenceMIM outperforms VAE models for text and is competitive with state-of-the-art auto-regressive approaches, including transformer-based models [], as measured by negative log-likelihood and perplexity. We further demonstrate the quality of the SentenceMIM representation by generating diverse samples around a given sentence and interpolating between sentences. Finally, we show the versatility of the learned representation by using SentenceMIM to solve a question answering task through text modelling alone, outperforming supervised baselines.

1. generative models for text data, with advantages:
- unsupervised learning with large corpora, 
- prob estimation, 
- filling-in/completion, ...
    
2. LVMs for unsupervised learning with text data. advantages 
  - fixed length codes
  - natural clustering and structure of learned representations,
    esp for downstream tasks
  - robustness of prob methods
  - supports interpolation and perturbation
  - refer to vision where they have been very useful?
  - Sampling with diversity (as opposed to beam search)
  - Interpretable, steerable latent representation
  
3) But LVMs have not had much success (Yang, Bowman, etc)
  - explain some of the attempts.
  - and the prob with P.C.
  
4) We introduce a new LVM based on MIM, and show that it does work on text data.
   - explain properties of MIM that make it amenable
   - and summarize how well it works on language data and some of the experiments
   
5) Contributions
     - new LVM that 'works' on text
     - expt on 4 datasets with good PPL and NLL, BLEU scores, 
    good generation of text, downstream task with representation (YahooCQA), etc.
    
    
    
    
% \begin{table}[th]
%     \centering
%     \setlength{\tabcolsep}{0.5em} % for the horizontal padding
%     {\scriptsize
%     \renewcommand{\arraystretch}{1.2}% for the vertical padding
%         \begin{tabular}{l | p{16cm}}
%         \hline \hline
%         \multicolumn{2}{l}{sMIM (1024) \textsuperscript{\textdagger}}   \\
%         \hline \hline
% (Q) & \textsc{<SOS>} when did cyril emmanuel king die ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i die in the heart of persia \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what is the king of a die ? i couldn't find a similar image \textsc{<EOS>} \\
% (A) long & \textbullet ~  die in the heart of a bad axe , but most importantly are scared to die . i have a hard drive \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} if e = mc squared , what is equal to mc cubed ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i think that = mc \^{} 2 \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i think the main characters here is the formula \textsc{<EOS>} \\
% (A) long & \textbullet ~ mc = mc , mc ? the formula is a good example of the noble gases . i think you'd are used \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} what are the backpacks that only have one strap that goes across your chest called ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ please help ! ! \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what goes your chest is called one that is used in the chest . i hope that \textsc{<EOS>} \\
% (A) long & \textbullet ~ your chest goes down in a chest that is known as the one i think of your chest . hope that helps \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} whats wrong with yahoo pool ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ what type of pool ? i think \textsc{<EOS>} \\
% (A) medium & \textbullet ~ whats wrong with the pool , and what are your favorite places . \textsc{<EOS>} \\
% (A) long & \textbullet ~ whats wrong with the pool of yahoo ! what are you wrong ? i liked the pool \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} why can girls be so complicated ( no offense girls ) ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ girls are currently looking for a video game \textsc{<EOS>} \\
% (A) medium & \textbullet ~ girls are so good that girls will be able to find out of the girls \textsc{<EOS>} \\
% (A) long & \textbullet ~ girls are so complicated that girls will be released in the heart of girls ? i hope this helps =) \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} do your co-workers drink on the job ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ what is the job ? i drink whisky \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what do you think ? i drink whisky the job and go through \textsc{<EOS>} \\
% (A) long & \textbullet ~ what do you drink ? the job of thumb , and i think they are a decent job \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} why is there no cure for hiv or other viruses ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ viruses ? i think it's too hot \textsc{<EOS>} \\
% (A) medium & \textbullet ~ no cure , no viruses of viruses . i think it's a good question \textsc{<EOS>} \\
% (A) long & \textbullet ~ no cure or no viruses ? i think the main reason for viruses is that the viruses in question will heal \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} when was the marine corp first started ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ first started in marine , and it was freezing \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what started the marine corps ? i think about the marine raider \textsc{<EOS>} \\
% (A) long & \textbullet ~ i started in the marine corps of marine , but they are very good and accurate . here's a marine corps \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} may you give me some investigatory projects about biology ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i have a clue of fish and meat \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i have a lot of projects , and i think about a minute surface \textsc{<EOS>} \\
% (A) long & \textbullet ~ i have a lot of projects in the philippines , and i think its a good resource for a human consumption \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} how do pain pills work on our pain ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ work on the surface i think \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i think it is a pain reliever , and i will definitely reccomend \textsc{<EOS>} \\
% (A) long & \textbullet ~ work pain . i think the pain of your heart is too bad for those who want to absorb \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} probability ratios ?\\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ what type of probability ? i \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what is the probability of a new object ? i used to predict \textsc{<EOS>} \\
% (A) long & \textbullet ~ what is the probability of a new year ? i mean , they are open to the surface tension \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} can you get pregnant while taking birth control pills ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i think the birth control \textsc{<EOS>} \\
% (A) medium & \textbullet ~ birth control pills , and i think it's just a good source \textsc{<EOS>} \\
% (A) long & \textbullet ~ i think that birth control pills are the main ingredient in your vagina . i will definitely use it \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} why are girls always so moody \& take things so personally ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ personally i hope so bad things are girls \textsc{<EOS>} \\
% (A) medium & \textbullet ~ personally i personally think so ... im looking for a new type of girls \textsc{<EOS>} \\
% (A) long & \textbullet ~ personally , things are so bad . i personally think of a new girl . it helps through girls and helps \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} what does it mean when your left ear itches really bad ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ bad ear plugs . it's not bad \textsc{<EOS>} \\
% (A) medium & \textbullet ~ bad ear , and i think it's a bad thing to hang \textsc{<EOS>} \\
% (A) long & \textbullet ~ it is a good ear to a couple of people , and i hope that helps =) \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} where should i play hockey at ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ hockey pucks . it's not bad \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i play the hockey team , but i think it's a good sport \textsc{<EOS>} \\
% (A) long & \textbullet ~ i play hockey for the hockey team , but i think it's a good idea to play hockey \textsc{<EOS>} \\
%         \hline 
% \end{tabular}
%     }
%     \caption{
%     Question and sampled answers from model sMIM (1024) \textsuperscript{\textdagger}
%     (\ie, trained on Everything dataset). 
%     We provide short/medium/long sampled answers (A) for each question (Q).
%     }
%     \label{tab:nlp-qa-everything-1}
% \end{table}


==> 2021-04-21 - SentenceMIM/tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


==> sections/ack.tex <==
% Acknowledgements should only appear in the accepted version.
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.


==> sections/intronotes.tex <==
Generative modelling of text has become one of the predominant approaches to natural language processing (NLP), particularly in the machine learning community. It is favoured because it allows for probabilistic reasoning, provides a principled learning framework (maximum likelihood). Unlike computer vision, where a variety of generative approaches have proliferated [], current methods for text mainly rely on auto-regressive models.

As an alternative, the family of generative latent variable models (LVMs), particularly variational auto-encoders (VAEs) [], have been successfully applied to many other domains. LVMs are widely studied because they can generate a latent representation that carries many useful properties. These are encoded as fixed-length vectors that capture salient semantic information, allowing for semantic comparison, interpolation, and search. They are often more interpretable, capturing distinct factors of variation in different latent dimensions. These properties have made LVMs especially compelling in the vision community [].

Despite their desirable qualities, LVMs have not enjoyed the same level of success in text modelling. There have been several proposals in recent years to adapt VAEs to text [], however these have not reached the same level of performance on natural language benchmarks as auto-regressive approaches. This is mainly attributed to the phenomenon of posterior collapse. A VAE consists of an encoder that maps data to a latent representation, and a decoder that maps the latent representation to data. In the case of posterior collapse, the decoder captures all of the modelling power and the encoder ends up conveying little to no information. For text, where the decoder itself is typically auto-regressive, this has proven challenging to mitigate.

In this paper, we introduce a new LVM for text based on the mutual information machine (MIM) framework [] called SentenceMIM. MIM is a recently introduced LVM framework that shares the same underlying architecture as a VAE, but uses a different learning objective that is more robust against posterior collapse. MIM learns a highly informative and compressed latent representation and often strictly benefits from more powerful architectures. VAE evaluation involves estimating a lower bound on the model log-likelihood called the evidence lower bound, or ELBO. Here, we propose an novel bound on the model log-likelihood for evaluating MIM models.

We show on four challenging datasets that SentenceMIM outperforms VAE models for text and is competitive with state-of-the-art auto-regressive approaches, including transformer-based models [], as measured by negative log-likelihood and perplexity. We further demonstrate the quality of the SentenceMIM representation by generating diverse samples around a given sentence and interpolating between sentences. Finally, we show the versatility of the learned representation by using SentenceMIM to solve a question answering task through text modelling alone, outperforming supervised baselines.

1. generative models for text data, with advantages:
- unsupervised learning with large corpora, 
- prob estimation, 
- filling-in/completion, ...
    
2. LVMs for unsupervised learning with text data. advantages 
  - fixed length codes
  - natural clustering and structure of learned representations,
    esp for downstream tasks
  - robustness of prob methods
  - supports interpolation and perturbation
  - refer to vision where they have been very useful?
  - Sampling with diversity (as opposed to beam search)
  - Interpretable, steerable latent representation
  
3) But LVMs have not had much success (Yang, Bowman, etc)
  - explain some of the attempts.
  - and the prob with P.C.
  
4) We introduce a new LVM based on MIM, and show that it does work on text data.
   - explain properties of MIM that make it amenable
   - and summarize how well it works on language data and some of the experiments
   
5) Contributions
     - new LVM that 'works' on text
     - expt on 4 datasets with good PPL and NLL, BLEU scores, 
    good generation of text, downstream task with representation (YahooCQA), etc.
    
    
    
    
% \begin{table}[th]
%     \centering
%     \setlength{\tabcolsep}{0.5em} % for the horizontal padding
%     {\scriptsize
%     \renewcommand{\arraystretch}{1.2}% for the vertical padding
%         \begin{tabular}{l | p{16cm}}
%         \hline \hline
%         \multicolumn{2}{l}{sMIM (1024) \textsuperscript{\textdagger}}   \\
%         \hline \hline
% (Q) & \textsc{<SOS>} when did cyril emmanuel king die ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i die in the heart of persia \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what is the king of a die ? i couldn't find a similar image \textsc{<EOS>} \\
% (A) long & \textbullet ~  die in the heart of a bad axe , but most importantly are scared to die . i have a hard drive \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} if e = mc squared , what is equal to mc cubed ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i think that = mc \^{} 2 \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i think the main characters here is the formula \textsc{<EOS>} \\
% (A) long & \textbullet ~ mc = mc , mc ? the formula is a good example of the noble gases . i think you'd are used \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} what are the backpacks that only have one strap that goes across your chest called ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ please help ! ! \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what goes your chest is called one that is used in the chest . i hope that \textsc{<EOS>} \\
% (A) long & \textbullet ~ your chest goes down in a chest that is known as the one i think of your chest . hope that helps \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} whats wrong with yahoo pool ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ what type of pool ? i think \textsc{<EOS>} \\
% (A) medium & \textbullet ~ whats wrong with the pool , and what are your favorite places . \textsc{<EOS>} \\
% (A) long & \textbullet ~ whats wrong with the pool of yahoo ! what are you wrong ? i liked the pool \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} why can girls be so complicated ( no offense girls ) ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ girls are currently looking for a video game \textsc{<EOS>} \\
% (A) medium & \textbullet ~ girls are so good that girls will be able to find out of the girls \textsc{<EOS>} \\
% (A) long & \textbullet ~ girls are so complicated that girls will be released in the heart of girls ? i hope this helps =) \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} do your co-workers drink on the job ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ what is the job ? i drink whisky \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what do you think ? i drink whisky the job and go through \textsc{<EOS>} \\
% (A) long & \textbullet ~ what do you drink ? the job of thumb , and i think they are a decent job \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} why is there no cure for hiv or other viruses ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ viruses ? i think it's too hot \textsc{<EOS>} \\
% (A) medium & \textbullet ~ no cure , no viruses of viruses . i think it's a good question \textsc{<EOS>} \\
% (A) long & \textbullet ~ no cure or no viruses ? i think the main reason for viruses is that the viruses in question will heal \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} when was the marine corp first started ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ first started in marine , and it was freezing \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what started the marine corps ? i think about the marine raider \textsc{<EOS>} \\
% (A) long & \textbullet ~ i started in the marine corps of marine , but they are very good and accurate . here's a marine corps \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} may you give me some investigatory projects about biology ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i have a clue of fish and meat \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i have a lot of projects , and i think about a minute surface \textsc{<EOS>} \\
% (A) long & \textbullet ~ i have a lot of projects in the philippines , and i think its a good resource for a human consumption \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} how do pain pills work on our pain ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ work on the surface i think \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i think it is a pain reliever , and i will definitely reccomend \textsc{<EOS>} \\
% (A) long & \textbullet ~ work pain . i think the pain of your heart is too bad for those who want to absorb \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} probability ratios ?\\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ what type of probability ? i \textsc{<EOS>} \\
% (A) medium & \textbullet ~ what is the probability of a new object ? i used to predict \textsc{<EOS>} \\
% (A) long & \textbullet ~ what is the probability of a new year ? i mean , they are open to the surface tension \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} can you get pregnant while taking birth control pills ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ i think the birth control \textsc{<EOS>} \\
% (A) medium & \textbullet ~ birth control pills , and i think it's just a good source \textsc{<EOS>} \\
% (A) long & \textbullet ~ i think that birth control pills are the main ingredient in your vagina . i will definitely use it \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} why are girls always so moody \& take things so personally ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ personally i hope so bad things are girls \textsc{<EOS>} \\
% (A) medium & \textbullet ~ personally i personally think so ... im looking for a new type of girls \textsc{<EOS>} \\
% (A) long & \textbullet ~ personally , things are so bad . i personally think of a new girl . it helps through girls and helps \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} what does it mean when your left ear itches really bad ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ bad ear plugs . it's not bad \textsc{<EOS>} \\
% (A) medium & \textbullet ~ bad ear , and i think it's a bad thing to hang \textsc{<EOS>} \\
% (A) long & \textbullet ~ it is a good ear to a couple of people , and i hope that helps =) \textsc{<EOS>} \\
%         \hline 
% (Q) & \textsc{<SOS>} where should i play hockey at ? \\
% \hdashline[1pt/1pt]
% (A) short & \textbullet ~ hockey pucks . it's not bad \textsc{<EOS>} \\
% (A) medium & \textbullet ~ i play the hockey team , but i think it's a good sport \textsc{<EOS>} \\
% (A) long & \textbullet ~ i play hockey for the hockey team , but i think it's a good idea to play hockey \textsc{<EOS>} \\
%         \hline 
% \end{tabular}
%     }
%     \caption{
%     Question and sampled answers from model sMIM (1024) \textsuperscript{\textdagger}
%     (\ie, trained on Everything dataset). 
%     We provide short/medium/long sampled answers (A) for each question (Q).
%     }
%     \label{tab:nlp-qa-everything-1}
% \end{table}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

